Neural Approaches to Entity-Centric Information Extraction

Artificial Intelligence (AI) has huge impact on our daily lives with applications such as voice assistants, facial recognition, chatbots, autonomously driving cars, etc. Natural Language Processing (NLP) is a cross-discipline of AI and Linguistics, dedicated to study the understanding of the text. This is a very challenging area due to unstructured nature of the language, with many ambiguous and corner cases. In this thesis we address a very specific area of NLP that involves the understanding of entities (e.g., names of people, organizations, locations) in text. First, we introduce a radically different, entity-centric view of the information in text. We argue that instead of using individual mentions in text to understand their meaning, we should build applications that would work in terms of entity concepts. Next, we present a more detailed model on how the entity-centric approach can be used for the entity linking task. In our work, we show that this task can be improved by considering performing entity linking at the coreference cluster level rather than each of the mentions individually. In our next work, we further study how information from Knowledge Base entities can be integrated into text. Finally, we analyze the evolution of the entities from the evolving temporal perspective.

==> definitions.tex <==
% List of Definitions
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\chapter*{List of Definitions}

\textbf{\newline\newline\Large Definitions concerning subject 1} \newline
\begin{acronym_expdlist}
\acro{DifficultWordA}{Explanation}
\end{acronym_expdlist}

\textbf{\newline\newline\Large Definitions concerning subject 2} \newline
\begin{acronym_expdlist}
\acro{DifficultWordB}{Explanation}
\end{acronym_expdlist}



% End of list of Definitions
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



==> klim_ch_temporal_el/old_manuscript.tex <==
\graphicspath{{klim_ch_temporal_el/figures/}}
\widowpenalty100000
\clubpenalty100000

% \documentclass[dvipsnames]{article}
% \documentclass{article}

% if you need to pass options to natbib, use, e.g.:
%     \PassOptionsToPackage{numbers, compress}{natbib}
% before loading neurips_data_2022

% ready for submission
% \usepackage{neurips_data_2022}

% to compile a preprint version, add the [preprint] option, e.g.:
%     \usepackage[preprint]{neurips_data_2022}
% This will indicate that the work is currently under review.

% to compile a camera-ready version, add the [final] option, e.g.:
%     \usepackage[final]{neurips_data_2022}

% to avoid loading the natbib package, add option nonatbib:
%    \usepackage[nonatbib]{neurips_data_2022}

% Submissions to the datasets and benchmarks are typically non anonymous,
% but anonymous submissions are allowed. If you feel that you must submit 
% anonymously, you can compile an anonymous version by adding the [anonymous] 
% option, e.g.:
%     \usepackage[anonymous]{neurips_data_2022}
% This will hide all author names.

% \usepackage[utf8]{inputenc} % allow utf-8 input
% \usepackage[T1]{fontenc}    % use 8-bit T1 fonts
% \usepackage{hyperref}       % hyperlinks
% \usepackage{url}            % simple URL typesetting
% \usepackage{booktabs}       % professional-quality tables
% \usepackage{amsfonts}       % blackboard math symbols
% \usepackage{nicefrac}       % compact symbols for 1/2, etc.
% \usepackage{microtype}      % microtypography
% \usepackage[table]{xcolor}         % colors
% \usepackage{graphicx}
% \usepackage{algorithm}
% % \usepackage{algpseudocode}
% \usepackage{algorithm,algpseudocode}
% \usepackage{multirow}
% \usepackage{amsmath}
% % \usepackage{ctable}
% \usepackage[inline,shorts]{enumitem}
% \usepackage{subcaption}
% %%%%%%% BEGIN added by TempEL
% \usepackage{makecell}

% \graphicspath{{figures/}}

% \algnewcommand{\LeftComment}[1]{\Statex \(\triangleright\) #1}

% \newcommand{\revklim}[1]{\textcolor{RoyalBlue}{#1}}
% \newcommand{\hideme}[1]{\textcolor{RoyalBlue}{}}
% \newcommand{\lucie}[1]{\textcolor{violet}{#1}}
% \newcommand{\etc}{etc.\ }
% \newcommand{\eg}{e.g., }
% \newcommand{\cf}{cf.\ }
% \newcommand{\ie}{i.e., }
% \newcommand{\vs}{vs.\ }
% \newcommand{\figref}[1]{Fig.~\ref{#1}}    % within sentence
% \newcommand{\figsref}[2]{Figs.~\ref{#1}--\ref{#2}}    % within sentence
% \newcommand{\Figref}[1]{Figure~\ref{#1}}  % start of sentence
% \newcommand{\Figsref}[2]{Figures~\ref{#1}--\ref{#2}}    % start of sentence
% \newcommand{\tabref}[1]{Table~\ref{#1}}
% \newcommand{\Tabref}[1]{Table~\ref{#1}}
% \newcommand{\Algref}[1]{Algorithm~\ref{#1}}
% \newcommand{\secref}[1]{Section~\ref{#1}}
% \newcommand{\equref}[1]{Eq.~(\ref{#1})}
% \newcommand{\eqsref}[2]{Eq.~(\ref{#1})--(\ref{#2})}
% \newcommand{\appref}[1]{\ref{#1}} 


% \definecolor{deepcarmine}{rgb}{0.66, 0.13, 0.24}
% \colorlet{negative0001}{deepcarmine!75}
% \colorlet{negative001}{deepcarmine!50}
% \colorlet{negative01}{deepcarmine!25}

% \definecolor{darkspringgreen}{rgb}{0.09, 0.45, 0.27}
% \colorlet{positive0001}{darkspringgreen!75}
% \colorlet{positive001}{darkspringgreen!50}
% \colorlet{positive01}{darkspringgreen!25}


% \DeclareMathOperator*{\argmax}{arg\,max}
% \DeclareMathOperator*{\argmin}{arg\,min}

%%%%%%% END

\hyphenation{}



% \title{TODO}

% The \author macro works with any number of authors. There are two commands
% used to separate the names and addresses of multiple authors: \And and \AND.
%
% Using \And between authors leaves it to LaTeX to determine where to break the
% lines. Using \AND forces a line break at that point. So, if LaTeX puts 3 of 4
% authors names on the first line, and the last on the second line, try using
% \AND instead of \And before the third author name.
\chapter[Temporal Entity Linking]{{\ourdataset}: Linking Dynamically Evolving and\\ Newly Emerging Entities}
% \title{{\ourdataset}: Linking Dynamically Evolving and\\ Newly Emerging Entities}
\label{chap:temporal_el}


\renewcommand\evenpagerightmark{{\scshape\small Chapter \arabic{chapter}}}
\renewcommand\oddpageleftmark{{\scshape\small Temporal Entity Linking}}

\renewcommand{\bibname}{References}

\begin{flushright}
% ---Rihanna, 2007
\end{flushright}

\noindent 

\emph{In this chapter we go one step further and analyze the evolution of the entities from temporal perspective. In order to achieve this, we create a new dataset which consists of 10 yearly snapshots of Wikipedia entities from 2013 until 2022. We further study how \textit{entity linking} task is affected by \begin{enumerate*}[(i)]
    \item changes of existing entities in time, and 
    \item creation of new emerging entities.
\end{enumerate*}. Furthermore, we do not restrict our analysis to the realm of \textit{named entities}, but incorporate all existing entities and concepts defined in Wikipedia. Our analysis showcases a continual decrease of performance in time, indicating that the entities from later versions of Wikipedia are harder to disambiguate than entities from earlier versions. Additionally, we demonstrate that the decrease in performance is specially sharp for entities requiring additional new knowledge (\eg new entities related to COVID-19 pandemic) for which the model was not pre-trained.}
\begin{center}
\par{$\star\star\star$}
\end{center}
\vspace{0.15in}

\par{\noindent\large{\textbf{K.~Zaporojets, L.A.~Kaffee, J.~Deleu, T.~Demeester, C.~Develder and I. Augenstein}}}
\vspace{0.1in}
\par{\noindent\textbf{In Submission.}}
\vspace{0.15in}


\par{\noindent\bf{Abstract}}
We live in a constantly evolving world where the % information on 
    entities surrounding us 
    % is constantly changing 
    are constantly changing,
    and new previously non-existing entities appear. 
    % In this paper we consider entity disambiguation task in a diachronic setting. 
    In this work, we study how this evolutionary scenario impacts the performance of a well established \textit{entity linking} task. 
    We introduce \ourdataset, entity linking dataset which consists of 10 yearly Wikipedia snapshots from 2013 to 2022, each one 
    composed of a set of \textit{anchor mentions} mapped to \textit{target entities} 
    of that year.
    % of entities and mentions. 
    %  and mentions to be linked to these entities
    This newly introduced 
    % dataset 
    resource
    contrasts with currently 
    % well established 
    existing
    entity linking 
    datasets 
    % data collections
    composed 
    % by 
    % mentions 
    % temporally 
    of
    fixed mentions linked to a
    % a links annotated using a 
    single static version of a target Knowledge Base (\eg Wikipedia 2010 for CoNLL-AIDA). 
    Conversely, for each of the temporal snapshots, \ourdataset~contains 
    % mentions that are linked 
    links 
    to both
    % both already existing 
    % both entities that are 
    % both 
    entities that are \textit{shared} across all of 
    % the temporal snapshots
    the years
    % (\textit{shared}) 
    as well as 
    % mentions linked to 
    completely \textit{new}, emerging entities.
    % , previously non-existing 
    % target entities. 
    This allows us to study 
    \begin{enumerate*}[(i)]
        \item how temporal evolution in the description of entities and mentions' contexts affects the performance of current models, and 
        \item compare it to that of completely new, previously non-existing entities of each of the time periods. 
    \end{enumerate*}
    Our experimental results show a significant temporal deterioration in performance (accuracy score) of up to -4.6\% for shared and up to -15.4\% 
    % accuracy@64
    % accuracy score 
    for new entities. This highlights the challenge of the introduced \ourdataset~dataset and opens new research prospects in the area of time-evolving entity disambiguation.  
    
  % The abstract paragraph should be indented \nicefrac{1}{2}~inch (3~picas) on
  % both the left- and right-hand margins. Use 10~point type, with a vertical
  % spacing (leading) of 11~points.  The word \textbf{Abstract} must be centered,
  % bold, and in point size 12. Two line spaces precede the abstract. The abstract
  % must be limited to one paragraph.
% \end{abstract}


\section{Introduction}
% Figure 1: TODO figure that would have:
%  - An cherry picked example of both anchor mention context as well as target entity evolution in time. 
%  - The example has to be very well known (ex: Donald Trump, but better not such controversial, better some more neutral topic). 
%  - The example has to make it clear that with the original context and entity definition, it would be hard to disambiguate with current context/entity definition
%  - The example has to make it clear that we also study the appearance of NEW entities in time, not only evolution of existing ones. 
% Paragraph 1: entity disambiguation as a very important task, yet only on a single version of the KB, we one step further; multiple target kb/kg. 
% - TODO: also include the difference between shared and new entities, using the examkple. 
% Entity disambiguation is a well established task that has attracted a lot of attention in scientific community. 
% We live in a constantly evolving world.... 
% In the current work we follow the common practice of \textit{``Wikification''} \cite{cheng2013relational,milne2008learning} where entity linking is done to Wikipedia KB.
Entity linking (EL) is a well established task which consists in mapping the anchor \textit{mentions} in text to target \textit{entities} that 
% denote 
describe
them in a Knowledge Base (KB) (\eg Wikipedia).\footnote{Some of the related work \cite{ganea2017deep, sevgili2020neural, kolitsas2018end, zhang2021entqa} distinguishes between \textit{entity disambiguation} and \textit{entity linking} tasks. This latter including \textit{mention detection} and \textit{disambiguation} in an end-to-end setting. In the current work, we follow a more conservative 
% entity linking task definition
naming convention 
\cite{wu2019zero, logeswaran2019zero, raiman2022deeptype, onoe2020fine, rao2013entity}, and use the term \textit{entity linking} and \textit{entity disambiguation} interchangeably.}
% ... the identifying the most suitable entity from Knowledge Base (KB) that defines a given \textit{anchor mention} in text.
% Recent models use both textual (\eg Wikipedia) (REF) as well as graph-based (\eg Wikidata) (REF), or complementary (REF bootleg) information from target knowledge bases to disambiguate. State-of-the-art architectures have achieved super-human performance (REF raiman). 
% The mainstream research [REF] is directed towards linking a fixed set of annotated mentions using a single version of target KB.
The mainstream datasets \cite{usbeck2015gerbil,roder2018gerbil} are composed of a fixed set of annotated mentions linked to a single version of target KB.
% , oblivious to the temporal evolution of a particular target KB or context of the anchor mentions.
% can experience. 
This static setup is oblivious to the inherently non-stationary nature of the entity linking task where both, target entities as well as anchor mentions change with time. The example in \figref{ch_temporal_el:fig:el_introduction} illustrates this time-evolving essence of entity linking with a simple evolutionary comparison between Wikipedia 2013 and 2022. It showcases two scenarios studied in the current paper: \begin{enumerate*}[(i)]
    \item temporal evolution of existing (\textit{shared}) entities across temporal cuts, and
    \item appearance of \textit{new}, previously non-existent entities
\end{enumerate*}. 
% Thus, 
% in the showcased example in \figref{ch_temporal_el:fig:el_introduction}, 
Concretely,
the description of \textit{shared} entity \textit{The Assembly} differs between Wikipedia 2013 and 2022. Furthermore, the context of mention ``Mejlis'' referring to \textit{The Assembly} also changes with time. Conversely, the \textit{new} entity \textit{Janssen COVID-19 vaccine} is introduced in 2021 with the corresponding mentions (\eg ``Johnson \& Johnson'' in \figref{ch_temporal_el:fig:el_introduction}) that are linked to it. 
% This time-evolving scenario presents a dual challenge to the current state-of-the-art models of both dealing with temporal drift in existing entities, as well as being able to incorporate the knowledge on newly introduced entries in the KB. 
% new previously non-existing entities appear in later versions of Wikipedia (in \figref{ch_temporal_el:fig:el_introduction}). 
% the problem by focusing where, target entities as well as anchor mentions evolve with time. 
% and not accounting for the evolution of entities in time.
% Intro with illustrative figure... Nice figure in \url{https://datasets-benchmarks-proceedings.neurips.cc/paper/2021/file/5737c6ec2e0716f3d8a7a5c4e0de0d9a-Paper-round2.pdf}

% Paragraph 2: we introduce a novel dataset that: 
%  anchor mentions in time 
%  target entities in time 
%  both wikipedia and wikidata 
%  10 cuts/snapshots
%  baselines 
%  evenly distributed temporal subsets
In this paper %, 
we introduce \ourdataset, a novel dataset whose goal is to capture this time-evolving characteristic of entity linking task. 
% the evolution of the anchor mentions and target entities of KB in time. 
In order to achieve this, we extract 10 equally spread \textit{yearly} snapshots (or cuts) from Wikipedia 
% and Wikidata 
entities starting from 01/01/\underline{2013} until 01/01/\underline{2022}. 
% Furthermore, 
We use each of these Wikipedia temporal snapshots to also extract anchor mentions with the surrounding text. This way, \ourdataset~captures 
the temporal evolution not only in target entities present in Wikipedia KB, but also in the context of anchor mentions linked to these entities. 
% the temporal evolution in both, the target entities in KB as well as the context of anchor mentions in text referring to these entities. 
Each of the 10 temporal snapshots of our dataset 
% is constituted by 
is composed of
training, test and validation sets with equal number of mentions and entities 
across the cuts. 
% and mentions per entity distribution. 
This way, we make sure that a possible difference in performance between temporal periods can 
%only be attributed to inherently time-evolving aspect 
be attributed exclusively to the evolution of textual content
% of Wikipedia 
and is not affected by dataset 
% variability 
distribution (\eg different sizes of training sets between snapshots) \revklim{[REF]}.
% such as the difference of training set sizes between snapshots. 
% and not to how the data is distributed in each of the temporal snapshots [REF to 2 or 3 similar temporal work]. 
Furthermore, we include in our dataset both mentions pointing to \textit{shared} entities across all of the studied temporal periods as well as to \textit{new} (emerging) entities inside a 
% particular 
given
temporal cut. 
% Furthermore, we downsample  This ... In order to make our snapshots evenly distributed we .... This way, the difference in performance.... 

% \Figref{ch_temporal_el:fig:el_introduction} illustrates the motivation behind our dataset... We observe how both, the \textit{anchor mention} context as well as the \textit{target entity} ``Title entity'' change between the snapshot 2013 and 2022. Additionally, new entities appear with the corresponding anchor mentions linked to them. This is the case of ``Title new entity'' with ``this completely new mention'' targeting it. 
% Paragraph 3: 
%  - non-trivial cases 
%  - 
% While Wikipedia is a popularly used textual source of mentions linked to entities (REF), it contains high bias towards \textit{trivial} disambiguation cases (REF). For example, our preliminary analysis shows that x\% of Wikipedia mentions can be successfully disambiguated by just matching the mention with the title of target page. Other y\% of mentions can be correctly linked by matching with the most likely entity with the highest prior \cite{guo2018robust}. 
% In order to avoid these biases,
% we exclude from \ourdataset~all the mentions that are
% \begin{enumerate*} [(a)]
%     \item identical to the title of the target pages (withing a pre-defined normalized edit distance score),
%     \item have the highest prior \cite{yamada2016joint} to the target page
% \end{enumerate*}. Furthermore, we make sure that there is no overlap of mentions between train, validation and test sets. This way, we expect to stimulate the creation of more robust entity linking models invariant to currently dominant biases such as mention-entity memorization
% \cite{wu2019zero,logeswaran2019zero,onoe2020fine} 
% and disambiguation towards most likely entities
% \cite{provatorova2021robustness,guo2018robust}. 
% We further downsample the number of mentions per entity to 10 in validation and test sets in order to avoid highly popular entities to dominate the final results (\ie popularity bias; REF).

% paragraph 4: 
% baseline 
% main analysis results 
% main contributions here or in 5th paragraph? 
Finally, as a baseline, we fine-tune and evaluate the bi-encoder component of BLINK model \cite{wu2019zero} on our newly introduced \ourdataset~dataset. 
Our experiments demonstrate
an increased temporal model deterioration for both shared (4.6\% accuracy points) as well as new (15.4\% accuracy points) entities. A more detailed analysis
% shows 
reveals
that the maximum drop in performance is observed for \textit{new} entities that require 
% completely new and 
fundamentally different world knowledge not present in the originally used corpus to pre-train BERT. 
% reveals that new entities requiring additional world knowledge not present in the originally pre-trained BERT model. 
% maximum drop in performance suffer new entities that require additional world knowledge, non-existent in the pre-trained BERT models. 
This is the case of COVID-19 related \textit{new} entities for which the bi-encoder model suffers additional deterioration of more than 22\% accuracy points compared to the rest of the new entities. 
% when comparing to the results on the first temporal snapshot.  
% \revklim{TODO RESULTS!!}. 
% Furthermore, our results show an even higher difference in performance (of up to 17\% accuracy points) for \textit{new} emerging entities that haven't been seen during fine-tuning and pre-training phases. 
% A more detailed analysis showcases that these general decrease in performance is accompanied with appearance of more granular and semantically similar candidates. 
% Furthermore, we showcase that new, emerging entities in Wikipedia not always require additional new knowledge to be disambiguated and therefore are not equally challenging. To prove this, we test with a subset of new entities that refer to completely unknown event during pre-training of our models: \textit{COVID pandemic}. We show that on these cases the model experiences a drop in performance of 12.5 \% accuracy points compared to the rest of \textit{new} entities.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Url to change the figure (made with diagrams.net): 
% https://app.diagrams.net/#G162Oo4yfIOezGe6dhm1K0pBQsa_G4w5hX
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[!t]
\centering
% left bottom right top
\includegraphics[width=0.7\columnwidth]{EL-examples}
%\caption{Introductory Example}
\caption{Illustration of KB entities changing over time: the Mejlis entity changes over time (both in its KB description and the contexts in which it is referenced to), while the Johnson \& Johnson vaccine is an entirely new one that did not exist before.}
\label{ch_temporal_el:fig:el_introduction}
\end{figure}
\section{Related Work}
% Table: Something nice here would be a table like Table 1 in \url{https://arxiv.org/pdf/2203.06823.pdf}. 
% Different categories of related work like in \url{https://datasets-benchmarks-proceedings.neurips.cc/paper/2021/file/4c56ff4ce4aaf9573aa5dff913df997a-Paper-round1.pdf}
% datasets described in 
\noindent\textbf{Entity Linking Datasets:} Entity linking has gained a lot of interest recently, becoming one of the most studied tasks in information extraction. Most of the current state-of-the-art models \cite{yamada2020global, orr2020bootleg, zhang2021entqa, de2021highly, de2020autoregressive} report on datasets presented under common GERBIL framework \cite{usbeck2015gerbil,roder2018gerbil}. This framework includes manually annotated datasets coming predominantly from news domain such as AIDA \cite{hoffart2011robust}, KORE50\cite{hoffart2011robust}, AQUAINT \cite{milne2008learning}, ACE2004, 
% (updated by \cite{guo2018robust}) 
 MSNBC \cite{ratinov2011local} and N$^3$ \cite{roder2014n3}. Other frequently used datasets from GERBIL include the web-based IITB \cite{kulkarni2009collective} and OKE 15/16 \cite{nuzzolese2015open}, as well as the tweet-based \cite{derczynski2015analysis}. Finally, 
 % GERBIL 
 this framework
 also covers larger, automatically annotated datasets such as WNED-WIKI and WNED-CWEB \cite{guo2018robust}. Even though GERBIL enables the use of multiple target knowledge bases (\eg Wikipedia, DBPedia, etc), it is limited to static annotations in the original datasets it covers. This contrasts with our newly introduced \ourdataset~dataset, where both the anchor mentions as well as target entity descriptions are taken from different time periods, enabling thus the study of temporal drift on performance of EL models. 
 % This stationary As a result it is  ..... are linked to a single version of ... This contrasts with \ourdataset..... 

More recently, the research interest has been shifting towards creating more niche entity linking datasets \cite{zaporojets2021consistent,zaporojets2021dwie, mohan2018medmentions,logeswaran2019zero} designed to 
% address the weaknesses in current EL evaluation resources, and 
stimulate the design of more robust disambiguation models. 
The most related to our work are the 
% recently introduced 
WikilinksNED \cite{onoe2020fine, eshel2017named} and ShadowLink \cite{provatorova2021robustness} datasets. 
% Similarly to WikilinksNED, \ourdataset~contains no overlap of mention-entity pairs between train, validation and test sets. 
WikilinksNED contains only unseen mention-entity pairs in its test subset, thus encouraging the design of models invariant to overfitting and memorization biases. 
Furthermore, ShadowLink contains \textit{overshadowed entities}: entities referred by ambiguous mentions whose most likely target entity is different.\footnote{For example, the anchor mention ``Michael Jordan'' linked to the scientist instead of to the 
% businessman and 
former basketball player.} We incorporate the challenges presented in WikilinksNED and ShadowLink in \ourdataset~(\ie by only considering overshadowed entity-mention pairs with no overlap between train, validation and test sets). This way, we intend to create a dataset containing \textit{non-trivial} cases with high degree of ambiguity \cite{guo2018robust}. 
% One line of research creates multi-task datasets where entity linking is annotated simultaneously with other tasks such as coreference resolution and relation extraction \cite{zaporojets2021consistent,zaporojets2021dwie, mohan2018medmentions}, motivating the creation of joint EL models. 
% Another branch of research is focused on creating datasets with more challenging evaluation scenarios. For example, \cite{onoe2020fine, eshel2017named} create WikilinksNED which contains only unseen mention-entity pairs in its test subset.
% \cite{logeswaran2019zero} go one step further and introduce a zero-shot entity linking (ZeShEL) dataset with target entities for each of the subsets (\ie train, validation and test) coming from different fandom \footnote{\url{https://www.fandom.com/}} wikis. 
 % \cite{provatorova2021robustness} construct ShadowLink and introduce the concept of \textit{overshadowed entities}: entities referred by ambiguous mentions whose most likely target entity is different (\eg the mention ``Michael Jordan'' referring to the scientist instead of to the businessman and former basketball player). 
 % The authors further demonstrate a drastic drop in performance of current state-of-the-art models on such overshadowed cases. We incorporate the challenges presented in WikilinksNED and ShadowLink in \ourdataset~(\ie by only considering overshadowed entity-mention pairs with no overlap between train, validation and test sets). This way, we intend to create a dataset containing \textit{non-trivial} cases with high degree of ambiguity \cite{guo2018robust}, stimulating a future research to address this more complex disambiguation scenario. 

% During the construction of \ourdataset we incorporate the challenges presented WikilinksNED and \cite{TODOrefSOMEBODYWHOTOOKPRIORLESSTHAN1ST}.  We achieve this by only incorporating less common mentions and avoiding overlap between mentions of different subsets. 
%%%%%%%%%%%% 
% To justify prior rank < 1 selection
% \cite{ilievski2018systematic} --> low prior justification head /tail
% \cite{guo2018robust} --> balanced prior probabilities
% \cite{provatorova2021robustness} --> overshadowing
% bootleg --> head/tail
% WikiDisamb30 \cite{ferragina2011fast} --> ambiguity --> TODO: read more in detail
% KORE50 (Hoffart 2012) --> ambiguity, long tail entities
%%%%%%%%%%%
% a dataset that similarly to \ourdataset~
% Similarly to \ourdataset, other datasets are built using already annotated Wikipedia mentions. 
% Thus \cite{ferragina2011fast} present Wiki-Disamb30 and Wiki-Annot30, two datasets that consist of fragments from Wikipedia of up to 30 tokens with annotated anchor mentions. 
% Other datasets such as OKE 15 \cite{nuzzolese2015open} use other web sources (\eg Web Data Commons, Common Crawl among others) to get annotated mentions. 
% (Ferragina and Scaiella, 2012) 
% Others are ... WNED-CWEB, WNED-WIKI \cite{guo2018robust} OKE 2015 \cite{nuzzolese2015open}. 
% TAC-KBP 
% group (with datasets ranging from the 2009 through 2012 competitions) 
% \cite{mcnamee2009overview}.... 
% Most recently, KILT \citet{petroni2020kilt} extended this .... as well as ... IITB dataset \cite{kulkarni2009collective} (part of GERBIL). 
 % propose to use a common GERBIL platform that allows a common evaluation framework for different scenarios including end-to-end and disambiguation only. Currently it includes datasets such as 
% Some of the datasets were cleaned and . ... 
% Most recently,    introduced KILT, an integrated dataset  ... ...
% Most recently, there has been interest in introducing datasets to address some of the challenges in entity linking. 
% Other more niche entity linking datasets such as zero-shot entity linking (ZeShEL; \cite{logeswaran2019zero}) and WikilinksNED that tackle entity linking in a zero-shot setting were introduced. 
% On the other hand, allows to evaluate entity disambiguation in a zero shot setting on entities unseen during training. 
% TODO: for zeshel maybe say that we are somewhat similar to it... 
% GERBIL: 37 new gold standard datasets, and 15 new annotators linking entities to any knowledge base
% While highly relevant, these datasets are monolithic in target knowledge base and anchor mentions, presenting a single snapshot (TODO: here clarify that mentions is different). While efforts such as X,Y (some efforts here on GERBIL) exist to link mentions from Z dataset to X knowledge base, they are limited to a very few knowledge bases and are not directed specifically to track the temporal evolution of target entities and are limited to anchor mentions present in the original text. 
% to the old mentions and do not allow to track the evolution in both entities and mentions for long periods of time... 
% We tackle this research gap by adding a temporal dimension to entity linking dataset. 
% We fill in this gap by creating a dataset where both the anchor mentions and the target entities are taken from different time periods (\ie snapshots) of Wikipedia. This enables research of entity linking in a temporal dimension where both target entities as well as the context of anchor mentions change in time. % TODO: 

% use a static version of target knowledge base and anchor text, ignoring the evolution of anchor context and target entities in time.  
% We provide temporal cuts for both wikipedia and wikidata KBs. 

% \noindent\textbf{Entity Linking and Disambiguation Models:} related work distinguishes \textit{entity linking} \cite{kolitsas2018end,de2020autoregressive,de2021highly, zaporojets2021consistent} that focus on both detecting and disambiguating entity mentions in text and \textit{entity disambiguation} \cite{ganea2017deep, wu2019zero} where the input mentions are given and the task is to disambiguate. In this work we focus on entity disambiguation by providing a dataset with mentions that have to be disambiguated to a given Knowledge Base (Wikipedia or Wikidata). The state-of-the art entity disambiguation models (REF) use a static version of target knowledge base and anchor text, ignoring the evolution of anchor context and target entities in time. We fill in this gap by providing a dataset where both the anchor mentions and the target entities are taken from different \textit{snapshots/cuts}. This enables research of entity linking in a temporal dimension where both entities and mentions change in time as well as new target entities appear.  
% \hideme{
% \revklim{\begin{enumerate}
%     \item main entity linking works: REF
%     \item main entity disambiguation works: REF
%     \item our contribution: temporal aspect , which requires learning new embeddings using traditional approaches (REF) and re-encoding using (REF). we use the re-encoding (bi-encoder) to show a temporal effect... 
%     \item \textit{Entity Linking} and \textit{Entity Disambiguation} as different concepts. We focus on Entity Disambiguation. Focus on temporal aspect. 
%     \item similar to zeshel work, but the entities can be seen, same entities in train/validation/test. However, similar to WikilinksNed(I think) , we use different surface forms.... Also similar as zeshel original paper that introduces it, where the focus is on mentions whose surface form differs substantially from the title (we also introduce the edit distance additionally to the categories in zeshel dataset work). 
%     \item TODO: there was another dataset (WikilinksNED?) where the authors on purpose removed the most likely entity to disambiguate. Check it , and indicate the similarity. 
% \end{enumerate}}}
% \noindent\textbf{Zero-Shot entity linking:} in order to make the disambiguation task more challenging
\textbf{Temporal Datasets:} the research on temporal drift in data has gained a lot of interest in the recent few years. The focus has been mostly on creating datasets to train language models on different temporal snapshots of corpus derived from scientific\cite{lazaridou2021mind}, newswire \cite{lazaridou2021mind,dhingra2022time}, Wikipedia \cite{jang2022temporalwiki}, and Twitter \cite{loureiro2022timelms} domains. 
% \cite{loureiro2022timelms, jang2022temporalwiki, dhingra2022time, rottger2021temporal,rosin2022time}. 
More recently, temporal datasets have appeared to address specific tasks such as sentiment analysis \cite{agarwal2021temporal, ni2019justifying, lukes2018sentiment}, text classification \cite{huang2018examining,he2018time}, named entity recognition \cite{rijhwani2020temporally,derczynski2016broad}, question answering \cite{lazaridou2021mind}, and entity typing \cite{luu2021time} among others. 
% bjerva2020back
% (REF), and truecasing \cite{rijhwani2020temporally} among others. 
% also emoticon detection by \cite{sogaard2021we}
However, the creation of datasets tackling the temporal aspect of entity linking has been largely left unexplored. 
% To the best of our knowledge the few exceptions tackling this issue are the work on \textit{emerging entities} \cite{derczynski2017results,farber2016emerging}. 
% In contrast, we extend this concept further by not only considering emerging entities, but change in entities across multiple cuts... 
To the best of our knowledge, the most related dataset to \ourdataset~is diaNED introduced by \cite{agarwal2018dianed}. The authors annotate mentions from historical documents that require additional temporal information from the context do be correctly disambiguated. Conversely, besides retrieving mentions from different temporal snapshots (\ie different Wikipedia versions), our main goal is 
to pair these mentions with the respective
% also include 
% different temporal versions 
% a number of 
time-evolving versions of target KB (\ie existing or new Wikipedia pages 
% that appear with time 
to which the extracted mentions are linked to). 
% focus on.... this differs to previous ones which focus on ``emerging new words'' \cite{lazaridou2021mind}... also these authors need to construct a synthetic QA dataset. 

% Also \cite{bjerva2020back}, \cite{del2019short}, \cite{jin2021lifelong}.
% aspect has been gaining interest to address specific tasks such as \cite{lazaridou2021mind,agarwal2021temporal,ehrmann2021named,rijhwani2020temporally, huang2018examining,fromreide2014crowdsourcing,ni2019justifying} demonstrate that.... 
% \revklim{(\textit{continual learning} and some datasets such as evolution of NER in time)}. 

% In contrast, we focus on  ... the main difference of entity disambiguation is that, being \textit{entity centric} it allows to trace both the target and anchor counter-parts referring to the same entity, this allows to zoom in on the exact knowledge location that possibly needs to be updated by the model... this differs to previous ones which focus on ``emerging new words'' \cite{lazaridou2021mind}... also these authors need to construct a synthetic QA dataset. 
% Also \cite{bjerva2020back}, \cite{del2019short}, \cite{jin2021lifelong}.

% machine translation: levenberg2010stream
% Exponential reservoir sampling for streaming language models.
% Dynamic language models for streaming text
% 
% \hideme{\revklim{\begin{enumerate}
%     \item TODO: check the dataset sent to Lucie/Isabelle at the beginning of the internship, maybe will lead to some other references as well (such as the models used). 
%     \begin{itemize}
%         \item Temporal Effects on Pre-trained Models for Language Processing Tasks \cite{agarwal2021temporal}
%         \item Mind the Gap: Assessing Temporal Generalization in Neural Language Models \cite{lazaridou2021mind}
%         \item TimeLMs: Diachronic Language Models from Twitter \cite{loureiro2022timelms}. 
%         \item TemporalWiki: A Lifelong Benchmark for Training and Evaluating Ever-Evolving Language Models \cite{jang2022temporalwiki}
%     \end{itemize}
%     \item Here also take into account how the following works will fit: \begin{itemize}
%         \item \cite{farber2016emerging}
%         \item Wikidated 1.0: An Evolving Knowledge Graph Dataset of Wikidata's Revision History \cite{schmelzeisen2021wikidated}
%         \item Discovering emerging entities with ambiguous names
%         \item Exploring Emerging Entities and Named Entity Disambiguation in News Articles
%         \item \textbf{diaNED: Time-Aware Named Entity Disambiguation for Diachronic Corpora} \cite{agarwal2018dianed}
%     \end{itemize}
% \end{enumerate}}}
% Knowledge-augmented models.... 
\textbf{Entity-Driven Datasets:} 
recent research has demonstrated the benefits of incorporating entity knowledge in various downstream tasks \cite{peters2019knowledge,yang2017leveraging,yamada2020luke,guu2020realm,verga2021adaptable,yasunaga2021qa,liu2022knowledge}.
% verga2020facts, % verlinden2021injecting,
% ,sun2018open
% such as language modeling (REF), question answering (REF), coreference resolution, relation extraction and named entity recognition \cite{verlinden2021injecting} to name a few. 
% TODO --> here check Severine's paper for more references. 
% Creation of datasets that allow to probe the entity-centric knowledge of such models has become of key interest. 
% This progress has been accompanied with creation of new entity-centric datasets. 
% For instance, REF introduces LAMA, a language model knowledge probing dataset .... 
% Others such as LAMA (REF),...(REF),... measure language model performance ...
% Some of the used datasets 
% used to test 
% the models' ability to identify and reason with entities include
% fall in the category of question answering, where the answers are derived from 
This progress has been accompanied by the creation of entity-driven datasets for tasks such as language modeling \cite{petroni2019language,agarwal2021knowledge,kassner2021multilingual}, question answering \cite{jiang2019freebaseqa,joshi2017triviaqa,yih2015semantic,lewis2021paq,saxena2021question}, fact checking \cite{onoe2021creak, aly2021feverous,thorne2018fever} and information extraction  \cite{yao2019docred,han2018fewrel,chen2018preco} to name a few. 
% others to site for information extraction: zaporojets2021dwie,zaporojets2021consistent, hoffart2011robust
% \cite{joshi2017triviaqa} introduces TriviaQA, a QA dataset where the answers are derived from entities or relations between entities in KB. Similarly, FreebaseQA (REF), WebQuestionsSP \cite{yih2015semantic} among others.... Other datasets intend to measure the model's ability to use entity information jointly with other information extraction tasks (\eg coreference resolution, entity linking, relation extraction, \etc) such as DWIE \cite{zaporojets2021dwie}, DocRED \cite{yao2019docred}.
% ... The models use datasets created using a specific spanshots... . 
% LAMA (REF),
Yet, recent findings \cite{fevry2020entities,lewis2020retrieval,verlinden2021injecting,heinzerling2021language,ri2021mluke,runge2020exploring}
% Also:
% peters2019knowledge
% onoe2021modeling
% ling2020learning
suggest that entity \textit{representation} and \textit{identification} 
(\ie identifying the correct entity that match a given text) 
are among the main challenges to increase the performance on such datasets. We expect that \ourdataset~can contribute in addressing this gap by 
\begin{enumerate*}[(i)]
\item encouraging research in finding more robust methods to creating \textit{entity representations} invariant to temporal changes, and 
\item improving entity identification for non-trivial scenarios involving ambiguous and uncommon mentions. 
\end{enumerate*}
% Furthermore, the \textit{non-trivial} characteristic of the mentions in our dataset (\ie surface form different from the title and not the most likely mention) presents a more challenging setup where current state-of-the-art models are more prone to fail \cite{provatorova2021robustness,logeswaran2019zero,wu2019zero}.
% can be used to train better entity representations and make the entity identification more robust and less dependent on a specific version of entity description.  

%such as question answering, coreference resolution, relation extraction, named entity disambiguation \cite{verlinden2021injecting}, among others has gained a lot of interest. This has \cite{petroni2019language} introduce LAMA, a dataset to test the.  entities play an important role in knowledge generation which can be beneficial for downstream tasks such as question answering \cite{fevry2020entities,verga2020facts,verlinden2021injecting}. 
% \cite{guu2020realm}, 
% \cite{fevry2020entities} showed how learning entity representations and correct entity identification can help downstream tasks such as question answering. ..., \cite{verga2020facts} on the other hand.... \cite{zhang2019ernie}?, \cite{peters2019knowledge}. Finally, works of \cite{verlinden2021injecting} demonstrate an incremental performance in tasks such as .... when injecting additional entity representations into the model. 
% Here the focus mostly on the \textit{closed-book} setting (mentioned in \cite{dhingra2022time} - check  salient span masking (SSM) here in both \textit{open-book} (Guu et al., 2020) and \textit{closed-book} settings (Roberts et al., 2020); \textit{cloze queries} used/cloze-style naturally follows SSM -  among others) where would be nice to teach the entity-centric models to memorize evolutionary entity-driven facts associated with anchor mentions. Currently the diachronic aspect is very little studied there. 

% \noindent\textbf{Entity Linking to KG vs Entity Linking to Wikipedia:}
% \revklim{\begin{enumerate}
%     \item (\textit{``Wikification''} \cite{cheng2013relational,milne2008learning})
%     \item traditionally, target knowledge bases based on text (...)
%     \item Lately more interest in KG.... and joint approach.
%     \item Driven by this need, we also include temporal cuts of wikidata in our dataset.... 
% \end{enumerate}}

% \noindent\textbf{Continual learning \& streaming LMs.} as in \cite{lazaridou2021mind}

% paragraph 1 entity disambiguation traditional models

% paragraph 2 continual learning and some datasets such as evolution of NER in time (I think it exists as far as I know). 

% paragraph 3 ...? maybe interaction of KB vs KG?? 

%\section{Dataset and Problem Definition}
\section{\ourdataset~Dataset}
In this section we will detail on how \ourdataset~was constructed (\secref{ch_temporal_el:sec:dataset_construction}), describing the main components of the creation pipeline (\figref{ch_temporal_el:fig:el_pipeline}).
% and pseudo-code (\Algref{ch_temporal_el:alg:dataset_builder}). 
Furthermore, we discuss the main aspects taken into account to guarantee the overall quality of our dataset (\secref{ch_temporal_el:sec:quality}). Finally, we present the statistics of \ourdataset~(\secref{ch_temporal_el:sec:dataset_statistics}), 
% that 
% underline 
% reveal
revealing its dynamically evolving nature. 
\subsection{Dataset construction}
\label{ch_temporal_el:sec:dataset_construction}
% Paragraph 1: 
%  1- source of data, overview of figure fig:el_pipeline with the main components
%  2- source of data, overview of figure fig:el_pipeline
% \revklim{Description of different components in dataset construction pipeline. Figure of the pipeline can be useful (like Fig 1 of \url{https://datasets-benchmarks-proceedings.neurips.cc/paper/2021/file/5878a7ab84fb43402106c575658472fa-Paper-round1.pdf})}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Url to change the figure (made with diagrams.net): 
% https://app.diagrams.net/#G162Oo4yfIOezGe6dhm1K0pBQsa_G4w5hX
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[!t]
\centering
\includegraphics[width=1.0\columnwidth, trim={0.0cm 0.0cm 0.0cm 0.0cm},clip]{el_copenhagen_pipeline_v12.pdf}
\caption{The Pipeline to create our \ourdataset~dataset. All the components are explained in \secref{ch_temporal_el:sec:dataset_construction}.}
\label{ch_temporal_el:fig:el_pipeline}
\end{figure}
% \Figref{ch_temporal_el:fig:el_pipeline} depicts the main components involved in the dataset creation. Next, we will describe each of the components individually along with the main aspects it tackles. 

\textbf{Snapshot Creator:} this module (see \figref{ch_temporal_el:fig:el_pipeline}) takes as input the Wikipedia history log dumps and outputs a number of elements for each of the yearly temporal cuts (\ie \textit{Elements per Cut} in \figref{ch_temporal_el:fig:el_pipeline}). First, it relies on \textit{Entity Filter} to \begin{enumerate*}[(i)]
    \item filter out pages that are irrelevant for our dataset (\ie categories, disambiguation pages, redirects and lists), and
    \item select the most stable version of 
    a Wikipedia page from the last month of the year in order to avoid introducing more volatile and potentially corrupted content edits (see \secref{ch_temporal_el:sec:quality}).
\end{enumerate*}
The second sub-component of Snapshot Creator is \textit{Entity Cleaner} and is used to strip the Wikipedia pages from wikitext markup content\footnote{\url{https://en.wikipedia.org/wiki/Help:Wikitext}}. We use both regular expressions as well as MediaWiki API for harder cases such as the interpretation of some of the wikitext templates (\eg the \texttt{Convert}\footnote{\url{https://en.wikipedia.org/wiki/Template:Convert}} template). Finally, the \textit{Mention Detector} sub-component 
% finds
detects 
the mentions in each of the Wikipedia entity pages. It also filters out mentions that point to anchors (\ie subsections in Wikipedia pages), pages in other languages than English,
% images or
files, red links (\ie links pointing to not yet existing Wikipedia pages) and redirects. 
% Next, it generates the \textit{Inverted Index} that allows to quickly identify Wikipedia pages where an anchor mention linked to a particular target entity can be found (see \ref{ch_temporal_el:dataset_builder} for more details on how it is used). 

As a result, the Snapshot Creator outputs \textit{Entity} and \textit{Mention Attributes}. These attributes are detailed in Appendix \ref{ch_temporal_el:app:mention_entity_attributes} and describe the main properties of entities (\eg content length in tokens, creation date, last modification date, etc.) and mentions (\eg edit distance between mention and title of target page, the mention prior, number of times a mention is linked to a particular target entity, etc.). 
% \begin{enumerate}
%     \item \textit{Mention Attributes}
% \end{enumerate}
Both mention and entity attributes form part of the final dataset, making it possible to perform additional analysis of the results (\eg study the performance of the models grouped by mention \textit{prior} attribute value). Furthermore, the Snapshot Creator creates the \textit{Inverted Index}, which allows to identify Wikipedia pages where an anchor mention linked to a specific target entity can be found (see 
% \ref{ch_temporal_el:dataset_builder}
the description \textit{Dataset Builder} further
for the details of how this index is used). Finally, the Snapshot Creator outputs the yearly temporal evolution of the textual content of each of the entities in the Wikipedia denoted as \textit{Entity Text} in \figref{ch_temporal_el:fig:el_pipeline}. This \textit{Entity Text} file also contains marked all the anchor mentions to be later extracted using \textit{Data Distributor} with the help of \textit{Inverted Index}. 

\textbf{Dataset Builder:} this component is responsible for the creation of the actual dataset given as input the \textit{Elements per Cut} produced by \textit{Snapshot Creator} (see above). The first step is to apply an additional \textit{Filter} to both entities and mentions. This filter intends to exclude mentions whose prior is the highest \cite{yamada2016joint} for a particular entity. More formally, a \textit{mention prior} is calculated as follows,  
    \begin{equation}
    P(e\vert m) = \vert A_{e,m} \vert / \vert A_{*,m} \vert \label{ch_temporal_el:eq:mention_prior},   
    \end{equation}
where $A_{e,m}$ is the set of links between anchor mention $m$ and target entity $e$, and $A_{*,m}$ is the set of links from anchor mention $m$. Additionally, the \textit{Filterer} excludes the mentions whose normalised edit distance from the target entity title is below established threshold.\footnote{During the generation of \ourdataset, we use the threshold of 0.2.} By ignoring the mentions with the highest prior and exact match with the title, 
we ensure that \ourdataset~contains non-trivial disambiguation cases where the naive approaches (\eg linking to the entity with the highest mention prior) would fail \cite{guo2018robust, logeswaran2019zero, wu2019zero, provatorova2021robustness}. % This also should motivate.... \revklim{I am here revising}
% This way, we eliminate the trivial cases where the mention can be disambiguated by matching with the title, which has been previously proved to make the disambiguation task more challenging \cite{wu2019zero,logeswaran2019zero}.
% make sure that naive \textit{prior} approaches based on linking the mention to the most likely entity \cite{guo2018robust} will fail and the model will have to perform additional disambiguation reasoning.
% \begin{enumerate}
%     \item \textit{Exclude mentions} whose prior is the highest \cite{yamada2016joint} for a particular entity. More formally, a mention prior is calculated as follows,  
%     \begin{equation}
%     P(e\vert m) = \vert A_{e,m} \vert / \vert A_{*,m} \vert \label{ch_temporal_el:eq:mention_prior},   
%     \end{equation}
%     where $A_{e,m}$ is the set of links between anchor mention $m$ and target entity $e$, and $A_{*,m}$ is the set of links from anchor mention $m$. By ignoring the mentions with the highest prior, we make sure that naive \textit{prior} approaches based on linking the mention to the most likely entity \cite{guo2018robust} will fail and the model will have to perform additional disambiguation reasoning. 

%     Additionally, the Filterer excludes the mentions whose normalised edit distance from the target entity is below established threshold\footnote{During the generation of \ourdataset, we use the threshold of 0.2.}. This way, we eliminate the trivial cases where the mention can be disambiguated by matching with the title, which has been previously proved to make the disambiguation task more challenging \cite{wu2019zero,logeswaran2019zero}.  
%     \item \textit{Exclude entities} whose length is below a defined threshold\footnote{We use 10 tokens}. This way, we avoid entities with very short and trivial descriptions. Furthermore, the entities that have less than 10 in-links (\ie number of mentions linked to them) are also filtered out. 
% \end{enumerate}
The second sub-component inside the Dataset Builder is \textit{Organiser}, and is responsible for grouping entities in two \textit{categories}: \begin{enumerate*}[(i)]
    \item \textit{new}, emerging and previously non-existent entities that are introduced in a particular snapshot, and
    % and previously non-existent entities in a particular snapshot, and 
    \item \textit{shared} entities across all the temporal snapshots. 
\end{enumerate*} The \textit{Organiser} also divides the mentions referring to a specific entity in different \textit{subsets} (\ie train, validation and test). 
% It imposes the constraint for normalised edit distance between the mentions in different subsets (\ie train, validation and test) referring to the same target entity be lower than 0.2. 
It constrains the normalized edit distance between mentions in different subsets (\ie train, validation and test) referring to the same target entity to be lower than 0.2. 
This way, we expect to discourage the potential models from memorizing the mapping between mentions and entities \cite{onoe2020fine}. 

The final sub-component of the Dataset Builder is \textit{Data Distributor}, which is responsible 
for equally distributing the data across all the temporal cuts. 
% that all the data across cuts is equally distributed. 
This way, the difference in performance can only be attributed to temporal evolution and not to 
% the differences 
inconsistencies
related to dataset variability (\eg different number of training instances in each of the temporal cuts). Concretely, we enforce that the number of \textit{shared} and \textit{new} entities as well as the number of mentions stays the same across the temporal snapshots (see \tabref{ch_temporal_el:tab:dataset_detail2}). 
% Concretely, we enforce an equal number of \textit{shared} and \textit{new} entities as well as the number of mentions across the cuts (see \tabref{ch_temporal_el:tab:dataset_detail}).
% In order to achieve this mention equality, we perform 
We achieve this by performing a random mention subsampling (in cuts with higher number of mentions) weighted by the difference of the number of mentions for each of the entities (sorted by the number of linked mentions) between the temporal cuts. This way, we 
% make sure that 
achieve a very similar
mention-entity distribution 
% is also very similar 
between the temporal snapshots 
% (see \figref{ch_temporal_el:fig:men_entity_distribution} in Appendix~\ref{ch_temporal_el:app:mention_per_entity_distribution}).
(see Appendix~\ref{ch_temporal_el:app:mention_per_entity_distribution}). 
Finally, the Data Distributor locates the filtered anchor mentions to extract in cleaned Wikipedia pages (\textit{Entity Text} in \figref{ch_temporal_el:fig:el_pipeline}) by using the \textit{Inverted Index} produced by the \textit{Mention Detector} sub-component of the \textit{Snapshot Creator}. It further pairs the context of each of the mentions with the respective content of target pages, producing this way the final \ourdataset~dataset. 
% for each of the temporal snapshots. 

% \subsection{Quality control}
\subsection{Quality Control} 
\label{ch_temporal_el:sec:quality}
\textbf{Corrupted Content:} Wikipedia is an open resource that relies on efforts of millions of Wikipedians to be extended (\revklim{REF?}). As such, its content is not always reliable, with errors due to human mistakes or intentional vandalism (\revklim{REF}). Despite numerous efforts to prevent the introduction of erroneous and misplaced content in Wikipedia (\revklim{REF}), 
% we have still detected many cases 
we have detected numerous cases
of corrupted 
% content 
entity descriptions
in the first version of our dataset. As a result, we adopted a simple, yet very effective heuristic: for each of the entities of a particular yearly snapshot, we select the most \textit{stable} (\ie the version of the entity that lasted the longest before being changed) content 
% of the entity pages 
of the last month of the year (December). Due to the fact that most of the corrupted content is rolled back very quickly, and even automatically by specialised bots (\revklim{REF}), this heuristic is very robust. We double checked the correctness of the extracted content by manually inspecting the temporal snapshots of top 100 entities whose textual description changed the most compared to the previous snapshot in \ourdataset~(we used Jaccard vocabulary similarity). 
% Through filtering (ex: min nr of inlinks, possibly min prior, max prior, ..., etc, ...). Manually controlled pages with highest jackard distance.

\textbf{Entity Relevance:} 
% we find it important that \ourdataset~includes entities with different level of popularity in order to avoid popularity bias (REF), including the tail entities \cite{orr2020bootleg,chen2021evaluating} with only a few anchor mentions pointing to them. 
we filter out entities that have less than 10 in-links (\ie number of mentions linking to the entity) or contain less than 10 tokens in its Wikipedia page in order to avoid including noisy content \cite{eshel2017named}. Additionally, in order to avoid evaluation bias towards mentions pointing to more popular entities during evaluation \cite{orr2020bootleg,chen2021evaluating}, we upper-cut the number of mentions per entity to 10 for our test and validation sets (see \figref{ch_temporal_el:fig:men_entity_distribution} in Appendix \ref{ch_temporal_el:app:mention_per_entity_distribution}). This way, 
we expect the accuracy scores to not be
% we ensure that the accuracy scores 
dominated by links to 
% more 
popular target entities (\ie entities with a big number of incoming links). 
% of anchor mentions pointing to them). % \revklim{also add the minimum entity length}

\textbf{Content Filtering:} in \ourdataset~we only consider mentions pointing to the main Wikipedia articles describing entities. The mentions pointing to anchors (subsections in a wikipedia document), images, files, and wiki pages in other languages are filtered out by our \textit{Snapshot Creator} component (see \figref{ch_temporal_el:fig:el_pipeline}). This component also ignores pages that are not Wikipedia articles (\eg files, information on Wikipedia users, etc.) as well as redirect pages. This way, both the target entities as well as anchor mentions in our dataset are obtained from a cleaned list of candidate pages referring to entities that contain a meaningful textual description in Wikipedia. 
% This way we ensure cleaned 
% We explicitly filter out entities Additionally the mentions linked to x,y,z are filtered inside the \textit{Entity Filter} sub-component of \textit{Snapshot Creator} (see \secref{ch_temporal_el:sec:dataset_construction}).
% the content of Wikipedia is not restricted to pages describing entities. It also contains elements such as categories, files, information on Wikipedia users, etc (REF). We filter out all the Wikipedia entities that are not main articles of Wikipedia (\eg files, information on users, media). 

% \revklim{wikipedia consists of .... entities such as categories etc ... similarly mentions.... our entity cleaner, and mention detector (is it here where links to anchors are filtered out??).} 

\textbf{Dataset Distribution:} during the construction of \ourdataset, we constrain the subsets to be of equal size and contain identical mention per entity distributions across all the temporal cuts (see Appendix \ref{ch_temporal_el:app:mention_per_entity_distribution}). This is implemented in \textit{Data Distributor} sub-component of the dataset creation pipeline (see \secref{ch_temporal_el:sec:dataset_construction} for further details). For example, the number of mentions in our training subset is 223,436 across all of the cuts (see \tabref{ch_temporal_el:tab:dataset_detail2} for further details). 
We argue that this setting will produce  uniform, structurally unbiased datasets across the cuts. This will allow to study exclusively the temporal effect on the performance of the models for each of the different time periods.  
Our reasoning is supported by previous work demonstrating that the size alone of the training set \cite{loureiro2022timelms} as well as different distribution of the number of mentions per entity \cite{orr2020bootleg} can significantly affect the performance of the final model. Furthermore, we do not constrain the total number of entities in the KB to be equal between time periods (see \figref{ch_temporal_el:fig:nr_wiki_entities}), since we consider it a part of the evolutionary nature of the entity linking task (\ie the temporal evolution of the target KB) we intend to study. 
% This way, the performance of the model
% We envision that this structural setup will provide a fair evaluation of different models, abstracting from the 
% it will provide a fair evaluation... from previous work on temporal evolution we know that the size alone of the training subsets used for fine-tuning can affect directly the performance of the final model on  \cite{loureiro2022timelms}. 
% a-growth in the number of mentions, as well as b-potentially different distribution of mentions per entities, implying difference in performance due to more (or less) average number of instances of mentions per entity \cite{orr2020bootleg}. Yet, we decide to keep the number of entities per wikipedia version untouched... because of what??? The component responsible for the dataset distribution is the \textit{Dataset Distributor} (see \figref{ch_temporal_el:fig:el_pipeline} and \secref{ch_temporal_el:sec:dataset_construction} for further details).

\textbf{Flexibility and Extensibility:} finally, we provide a framework that can be used to re-generate the dataset with different parameters as well as to extend it with newer temporal snapshots. 
% In  we include all possible hyperparameters that can be used to re-generate the dataset with different characteristics. 
This includes the option to re-generate a dataset with a 
% different 
customized
number of temporal snapshots (\eg quarterly instead of yearly spaced), different mention attributes (\eg filtering out by mention prior values), entity popularity (\eg filtering out entities that have more than a certain number of in-links), among others (see Appendix \ref{ch_temporal_el:app:hyperparameters} for a complete list). 

% \begin{enumerate}
%     \item min prior/max prior
%     \item min inlinks
%     \item filtering using the most stable version in the last month of the year (to deal with vandalism/corrupted versions). 
%     \item Mention diversity, entity diversity, non-overlapping entities.
%     \item Entities that have inlinks across different cuts, mean they are stable entities. 
%     \item highest edit distance manually controlled (TODO)
%     \item content length (at least 10 words?) of the target page in order to avoid pointing to empty pages. Ex: \texttt{Q16879410}
%     \lucie{\item Buckets with number of mentions per entity? Or already covered?}
%     \item diversity of the mentions, by scanning across mentions of different surface form, this makes it NOT biased towards the most popular mentions?. 
%     \item (maybe not here) on flexibility: the script allows to ``easily'' re-generate the dataset with different parameters (ex: total nr of entities, max number of mentions per entity) as well as to add new years. Also possible to change the temporal distance between the snapshots (in the current setup it is yearly, but can be monthly, daily, etc....). We can even generate different datasets such as \texttt{-base}, \texttt{-medium}, \texttt{-large}. 
% \end{enumerate}

% Pseudo-code sketched in \Algref{ch_temporal_el:alg:dataset_builder} \lucie{(if you keep the dataset distribution close to Wikipedia, if not dismiss) Real world setup, knowledge bases such as Wikipedia change to reflect changes in the real world. This includes an increase in number of entities, increase in content about an entity, and change of the context of terms established before}
% \revklim{Important to preserve the dataset distribution} 
% \textbf{Dataset Builder}
% it filters (\textit{entity filter}) out Wikipedia pages that are irrelevant
% \footnote{Downloaded from \url{https://dumps.wikimedia.org/enwiki/}}
% In order to make our dataset more challenging... we follow.... (\revklim{REF work in prior, there was another dataset with mentions with prior rank $>$ 1} ), edit distance, difference between mention and title as in \revklim{zeshel REF} and between mentions as in WikilinksNED \cite{eshel2017named, onoe2020fine}. \textit{Degree of ambiguity} based on prior \cite{guo2018robust}, focusing on overshadowed entities \cite{provatorova2021robustness, ilievski2018systematic}. This way, we expect that the introduced dataset will present a challenge to the current state-of-the art ... which will require additional reasoning in order to disambiguate given mentions.... Divide in buckets to study the head-tail effect similarly to \cite{orr2020bootleg}.  
% \subsection{Dataset statistics}

% \textbf{Snapshot/Cut Creator}
% % \begin{itemize}
% % \item Snapshot/Cut Creator: 
%     \begin{itemize}
%         \item Input: 
%         \begin{itemize}
%             \item \textit{Wikidata/Wikipedia history} logs: consists of compressed xml files with one entry for each of the temporal modifications in wikidata/wikipedia. % (terabytes of xml files). 
%             % \item \textit{Wikipedia history} logs. % (terabytes of xml files). 
%             % \item \texttt{page-info.sql} table to match wikipedia page ids with wikidata qids.
%             % \href{http://www.overleaf.com}{Something Linky}
%             \item \href{https://www.mediawiki.org/wiki/Manual:Page_props_table}{\textit{page\_props}} table (not in \figref{fig:el_pipeline}): table with properties that include the wikidata qid corresponding to each of the wikipedia pages. Currently is being replaced/complemented with \textit{sitelinks} element of each of the wikidata entities.
%         \end{itemize}
%         \item Processing: 
%         \begin{itemize}
%             \item \textit{Entity Filter}: 
%             \begin{enumerate}
%                 \item Ignores Wikipedia pages that are categories, disambiguation pages, redirects and lists. 
%                 \item Selects the most ``stable'' wikipedia/wikidata version (the one that lasted the longest) of the last month in order to avoid including corrupted content. 
%                 \item Matches a particular wikipedia page with wikidata entity using \texttt{page-props.sql} table. All the target pages are internally represented by wikidata qid and NOT wikipedia page title. \revklim{\textit{WIP:} implementing wikidata-wikipedia matching using wikidata \textit{sitelinks} attribute of each of the temporal cuts.}
%                 \item Tracks the \textit{title changes} of a particular page in time (so then can be matched to target links of mentions in each of the temporal cuts). \revklim{\textit{WIP:} implementing wikidata-wikipedia matching using wikidata \textit{sitelinks} attribute of each of the temporal cuts.}
%             \end{enumerate}
%             \item \textit{Mention detector:} using the filtered entities (previous point) 
%             \begin{enumerate}
%                 % \item Extracts mention information (anchor mention, target page) and page information (page creation date, page last modification date of the cut). 
%                 \item Filters out mentions: 
%                 \begin{itemize}
%                     \item Mentions pointing to anchors (sections inside a particular page),
%                     \item Mentions pointing to pages in other language than english,
%                     \item Mentions pointing to images and other files,
%                     \item Mentions pointing to redirects,
%                     \item Mentions pointing to red links (non-existent pages).
%                 \end{itemize}
%                 \item Builds \textit{inverted index}: a map for each of the snapshots that, given anchor mention $m$ and target entity $e$, returns the pages where this mention $m$ is linked to target $e$.
%                 \item  Extracts \textit{anchor mention attributes} for each of the snapshot (mention\_text, target\_wikidata\_qid, target\_wikipedia\_title, mention\_prior as defined in \cite{yamada2016joint}, prior\_rank, nr\_links, edit\_distance\_mention\_title, normalised\_edit\_distance\_mention\_title, overlap\_type as defined in \cite{logeswaran2019zero}, avg\_prior\_rank, avg\_prior, nr\_inlinks).
                
%                 % TODO: normalised edit distance formulation. 
                
%                 \textit{Mention prior} formulation. 
% \begin{equation}
%   P(e\vert m) = \vert A_{e,m} \vert / \vert A_{*,m} \vert \label{ch_temporal_el:eq:mention_prior},   
% \end{equation}
% where $A_{e,m}$ is the set of links between anchor mention $m$ and target entity $e$, and $A_{*,m}$ is the set of links from anchor mention $m$. 
                
%                 \revklim{TODO: entity prior formulation:}
% \revklim{                
% \begin{equation}
%   P(e) = \vert A_{e,*} \vert / \vert A_{*,*} \vert \label{ch_temporal_el:eq:entity_prior},
% \end{equation}}
% \revklim{where $A_{e,*}$ is the set of links to target entity $e$ and $A_{*,*}$ is the set of all links.}
% % Normalised edit distance: 
% % \revklim{                
% % \begin{equation}
% %   E(t_1,t_2) =  \label{ch_temporal_el:eq:normalised_edit_distance},
% % \end{equation}}
%                 \item Extracts \textit{target entity attributes} for each of the snapshot (page\_id, wikipedia\_title, wikidata\_qid, creation\_time, revision\_time, content\_length).
%             \end{enumerate}
            
%             % Regexes as well as wikipedia api (for templates such as ``Convert'' and ``SubatomicParticle'') are used here. 
%             \item \textit{Entity cleaner:} using filtered entities (first point)
%             \begin{enumerate}
%                 \item 
%             Wikipedia: Cleans the text from markups (\eg the infoboxes are removed). Leaves only text with mentions marked in it. 
%             \item Wikipedia: To interpret some of the wikipedia elements (\eg \textit{Convert} template), wikipedia API is invoked. 
%             \item Wikipedia: Removes some sections (ex: ``references'', ``see also'', ``notes'', ``external links''). 
%             \item Wikidata: leaves only \textit{triples} $\langle$subject, predicate, object$\rangle$ with labels and description only in english. Other values (\eg numbers) as well as elements such as \textit{references} are removed. 
%             \end{enumerate}
%         \end{itemize}
%         \item Output: 
%         \begin{itemize}
%             % \item \textit{Entity Filter}: 
%             % \begin{itemize}
%             %     \item \textit{Filtered target entities}: that are no categories, lists, disambiguation pages or redirect pages. 
%             %     \item \textit{The most stable version of wikipedia/wikidata entity} in the last month. 
%             % \end{itemize}
%             \item \textit{Mention detector}: for each of the filtered (by \textit{Entity Filter}) entities and mentions:  
%             \begin{itemize}
%                 % \item \textit{Filtered anchor mention}s: no mentions pointing to anchored links (sub-sections of a wikipedia page) or red links (non-existent pages).             
%                 \item \textit{Anchor mention attributes} for each of the snapshot (mention\_text, target\_wikidata\_qid, target\_wikipedia\_title, prior as defined in \cite{yamada2016joint}, prior\_rank, nr\_links, edit\_distance\_mention\_title, normalised\_edit\_distance\_mention\_title, overlap\_type as defined in \cite{logeswaran2019zero}, avg\_prior\_rank, avg\_prior, nr\_inlinks).
%                 \item \textit{Target entity attributes} for each of the snapshot (page\_id, wikipedia\_title, wikidata\_qid, creation\_time, revision\_time, content\_length).
%                 \item \textit{Inverted index}: a map for each of the snapshots that, given anchor mention and target entity, returns anchor pages the anchor mention can be found in.   
%             \end{itemize}
%             \item \textit{Entity cleaner}: 
%             \begin{itemize}
%                 \item \textit{Wikidata triples} for each of the entities of wikidata that have wikipedia page with snapshots for 2013-2022 years.
%                 \item \textit{Wikipedia text} (with and without marked mentions) of each of the pages of wikipedia with snapshots for 2013-2022 years. 
%             \end{itemize}
% %            \item \textit{Mention statistics} for each of the snapshot (mention\_text, target\_wikidata\_qid, target\_wikipedia\_title, prior as defined in \cite{yamada2016joint}, prior\_rank, nr\_links, edit\_distance\_mention\_title, normalised\_edit\_distance\_mention\_title, overlap\_type as defined in \cite{logeswaran2019zero}, avg\_prior\_rank, avg\_prior, nr\_inlinks). 
% %            \item \textit{Page statistics} for each of the snapshot (page\_id, wikipedia\_title, wikidata\_qid, creation\_time, revision\_time, content\_length). 
% %            \item \textit{Inverse dictionary} (given mention and target page, returns all the anchor pages the mention appears in); needed when creating dataset. 
% %            \item \textit{Properties (triples)} for each of the entities of wikidata that have wikipedia page with snapshots for 2013-2022 years. 
% %            \item \textit{Text} (with and without marked mentions) of each of the pages of wikipedia with snapshots for 2013-2022 years. 
%         \end{itemize}
%     \end{itemize}

%     \begin{itemize}
%         \item Input: 
%         \begin{itemize}
%             \item \textit{Mention attributes}: to get statistics such as \textit{prior} or edit distance to filter out ``easy'' cases.
%             \item \textit{Entity attributes}: such as \textit{creation date} to identify the ``new\_entities'' category of target entities that are new in a particular time cut (ex: entities whose wikipedia pages were created in 2014). 
%             \item \textit{Inverted index}: to identify the anchor pages where a mention pointing to a specific target entity can be found in. 
%             \item \textit{Wikipedia text}: to get the anchor context (the mention and text surrounding the mention) as well as target text. 
%             \item \textit{Wikidata triples}: % not used yet, we would need to include this when trying baselines that also rely on wikidata such as \cite{orr2020bootleg}. 
%         \end{itemize}
%         \item Processing:  
%         \begin{itemize}
%             \item \textbf{Filter}: performs additional fine-grained filtering of anchor mentions and target entities to build the dataset. 
%             \begin{itemize}
%                 \item Select \textit{target entities} that have at least 10 inlinks (mentions pointing to them), trying to avoid too noisy pages. 
%                 \item Select \textit{anchor mentions} with \textit{prior\_rank} stat for a particular target page is 2 or higher. This way a naive prior-based (linking to the most likely entity given a mention text) approach won't work: actual ``disambiguation'' has to be done. 
%                 \item Select \textit{anchor mentions} with at least 0.2 normalised edit distance (TODO eq. REF) to target wikipedia page title (so the model can not directly match mention with the title).  
%             \end{itemize}
%             \item \textbf{Organiser}: organises the dataset in categories (\textit{shared} and \textit{new\_entities}) and subsets (\textit{train}, \textit{validation} and \textit{test}):
%             % \item Across subsets (train, validation, test): 
%             \begin{itemize}
%                 \item All the target entities are shared between subsets (currently, a particular target entity is located in \textit{train}, \textit{validation}, and \textit{test} subsets). 
%                 \item The anchor mentions referring to a particular target entity have a minimum normalised edit distance of 0.2 between subsets (so the model can not exactly memorize a particular mention matching target page). 
%                 \item The target entities are organised in two types: \textit{shared} and \textit{new\_entities}. The \textit{shared} entities are shared across all the snapshots and allow to dynamic evaluation of performance as the content of a particular target entity changes in time. The \textit{new\_entities} are new entities in Wikipedia \revklim{and Wikidata} for a particular cut, and enable the evaluation of the performance on new entities that are unseen in previous cuts. 
%             \end{itemize}
%             \item \textbf{Data distributor}:
%             \begin{itemize}
%                 \item The target entities are divided in 4 \textit{buckets}, each one comprising entities with minimum and maximum number of anchor mentions linked to them. This way, the resulting dataset will contain both \textit{tail} (entities linked from few mentions) as well as \textit{head} (entities linked from many mentions) entities. 
%                 % so some target entities appear more times in training set (linked from 100 or more anchor mentions), and other entities appear only a few times (linked from 1 to 10 anchor mentions). 
%                 We hypothesise that some training algorithms might need more mention instances targeting a specific entity than others.  
%             \end{itemize}
%         \end{itemize}
%         \item \textit{Output}: currently the output is suited to train BLINK baseline \cite{wu2019zero} where each data point consists of the following fields: 
%         \begin{enumerate}
%             \item anchor\_context\_left: text to the left of anchor mention. 
%             \item anchor\_mention: text of the anchor mention. 
%             \item anchor\_context\_right: text to the right of anchor mention. 
%             \item target\_page: text of target page (first tokens including title). 
%             \item Attributes: 
%             \begin{itemize}
%                 \item total\_count\_mentions (how many times tha anchor mention is repeated in wikipedia)
%                 \item nr\_inlinks (nr of anchor mentions pointing to a particular target page)
%                 \item prior as dfined by \cite{yamada2016joint} (see \equref{ch_temporal_el:eq:mention_prior}). 
%                 \item prior\_rank 
%                 \item edit\_distance (anchor mention vs target page title)
%                 \item normalised\_edit\_distance (anchor mention vs target page title) % (see Eq...TODO)
%                 \item overlap\_type (as defined in \cite{logeswaran2019zero}) 
%                 \item avg\_prior\_rank of target page (the higher, the harder in average the page is to disambiguate). 
%                 \item avg\_prior of target page (the lower, the harder in average the page is to disambiguate).
%                 \item category (currently either ``shared'' or ``new\_entity''). 
%                 \item \revklim{TODO: entity prior (see \equref{ch_temporal_el:eq:entity_prior})}
%             \end{itemize}
%         \end{enumerate}
%         Currently, we are studying how to adapt the output for other models also relying on wikidata KG such as \cite{orr2020bootleg}. 
%     \end{itemize}

%%%%%%%%%%%%%%%%%%%%%%%%
% The python code of this pseudo-code located at: https://gitlab.ilabt.imec.be/kzaporoj/el_copenhagen/-/blob/main/src/wiki/wikipedia/jobs/dataset_creation/s03_final_dataset_creator_v2.py
%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{algorithm}
% \textbf{Input:} \vspace*{-2mm}
% \begin{enumerate}
%     \item $C \leftarrow \{2013, 2014, \ldots, 2022\}$ % CUTS
%     \item $S \leftarrow \{$train, validation, test$\}$ % SUBSETS
%     \item $B \leftarrow$ Buckets configuration (\revklim{TODO more details}) % BUCKETS 
%     \item $A(c) \leftarrow$ Anchor\ mentions\ linked\ to\ target\ entities + attributes for snapshot $c$ 
%     \item $W^{t}(c) \leftarrow$ wikipedia text for snapshot $c$
%     \item $W^{g}(c) \leftarrow$ wikidata triples for snapshot $c$ 
%     \item $\lambda \leftarrow$ constant ($0.2$) of minimum normalised edit distance
% \end{enumerate}\vspace*{-1mm}
% \textbf{Output:} dataset $D$
%   \begin{algorithmic}[1]
% \vspace{1mm}
% % \State TODO Other Initialize...\vspace*{1mm}
% \LeftComment{\textbf{Filter:} by attributes (\eg inlinks, edit distance anchor mention vs. target title, prior rank, etc. )}
% \State $T(c) \leftarrow \mathrm{filter\_attrs}(A(c)) \ \forall c \ \in C$\vspace*{1mm}
% \LeftComment{\textbf{Organiser:} divide in entity types (shared,new) for each cut/snapshot}
% \State $E(\mathrm{shared}, c) = t \in T(c) \colon t.\mathrm{entity} \in \{t'.\mathrm{entity}\ \forall t' \in T(c')\} \ \forall c' \in C$ % {other_cut \setminus cut}
% \State $E(\mathrm{new}, c) = t \in T(c) \colon t.\mathrm{entity} \notin \{t'.\mathrm{entity}\ \forall t' \in T(c')\} \ \forall c' \in C\setminus \{c\}$ % {other_cut \setminus cut}
% % \State $E(\mathrm{new}, c) = t \in T(c) \colon t \notin T(c') \ \forall \ c' \in C\setminus \{c\}$ % {other_cut \setminus cut}
% \vspace*{1mm}
% \LeftComment{\textbf{Organiser:} cluster mentions in \textit{subsets}: no two identical mentions linked to the same entity in different subsets of $S$}
% % \State TODO
% \For{$c$ \textbf{in} $C$}
% 	\For{$e \in \{E(\mathrm{shared}, c)\ \cup\ E(\mathrm{new}, c)\}$} 
% 		\State $M(e,c,s) \leftarrow \{m \in e.\mathrm{mentions}\} \colon \mathrm{edit\_dist}(m, m')>\lambda \  \forall m' \in M(e,*,s'\in\{S \setminus s\})$
% 	\EndFor
% \EndFor
% \vspace*{1mm}
% \LeftComment{\textbf{Data Distributor:} distribute data according to buckets configuration}
% \For{$b$ \textbf{in} $B$}
% \State $E'(b) \leftarrow \{e \in E(*,c) \colon \vert M(e,c,s) \vert > b.\mathrm{min\_mentions(s)} \ \forall s \ \in S, c \in C\}$
% \State $E'(b)  \leftarrow \mathrm{uniform}\big(E'(b), b.\mathrm{nr\_entities}\big)$
% \For{$e \in E'(b)$}
% \For{$c \in C$}
% \For{$s \in S$}
% \State $M (e,c,s,b) \leftarrow \mathrm{uniform\_m}\Big(M(e,c,s), \min\big(b.\mathrm{max\_mentions(s)}, \argmin\limits_{c'} M(e,c',s)\big)\Big)$
% \State $D.\mathrm{add}\big(m', e, c, s, \mathrm{inverse\_index}(m',e,W^{t}(c),W^{g}(c))\big) \ \forall m' \in M (e,c,s,b)$
% \EndFor 
% \EndFor 
% \EndFor
% \EndFor

%  \caption{Pseudo-code of \textit{Dataset Builder} component (see \figref{ch_temporal_el:fig:el_pipeline}).} \label{ch_temporal_el:alg:dataset_builder}
% \end{algorithmic}
% \end{algorithm}

\subsection{Dataset Statistics}
\label{ch_temporal_el:sec:dataset_statistics}
\tabref{ch_temporal_el:tab:dataset_detail2} summarizes the dataset statistics. 
% Following similar work in \revklim{REF}, 
We divide each of the temporal snapshots into train, 
validation and test subsets containing equal number of \textit{shared} and \textit{new} entities. The number of mentions differs between the subsets since we upper-bound to 10 the maximum number of mentions per entity in validation and test sets (see \textit{Entity Relevance} in \secref{ch_temporal_el:sec:quality} for additional details). Further statistics related to the distribution of the number of mentions per entity are illustrated in \figref{ch_temporal_el:fig:men_entity_distribution} of Appendix \ref{ch_temporal_el:app:mention_per_entity_distribution}. 
% in order for the metric to not be overly influenced by the most popular entities 
 % \Figref{fig:men_entity_distribution} illustrates the distribution of mentions per entity. Here we observe a long-tail phenomenon characterised by the majority of entities linked to by few mentions. Furthermore, all the data distributions are equal between the subsets we achieve this by performing a weighted sub-sampling of mentions across the snapshots. This way, we guarantee that any difference of performance across the cuts is only attributed to temporal evolution and not to other aspects related to data distribution (\eg more training data points in one cut compared to others, more \textit{tail} entities with less mention per entity, etc.). 

Additionally, we collect statistics related to temporal drift in content for both, the target entities (\figref{ch_temporal_el:fig:evolution_entities_jaccard} and \figref{ch_temporal_el:fig:evolution_entities_edistance}) as well as the context around the anchor mentions (\figref{ch_temporal_el:fig:evolution_mentions}). Concretely, \figref{ch_temporal_el:fig:evolution_entities_jaccard} illustrates Jaccard vocabulary similarity between the textual description of \textit{shared} entities in 2013 and posterior years of the across the temporal snapshots in \ourdataset. We observe a continual decrease, indicating that in average, the content of the entity description in Wikipedia is constantly evolving in terms of the used vocabulary. This is also supported by the graph in \figref{ch_temporal_el:fig:evolution_entities_edistance}, which 
% illustrates a constant 
showcases a continuous
temporal increase of the average value of normalised edit distance across \textit{shared} entities. Finally, in \figref{ch_temporal_el:fig:evolution_mentions} we 
showcase
% analyse
the temporal drift in the vocabulary (\ie Jaccard vocabulary similarity) of the context around the mentions pointing to a specific entity. We find it experiences a more significant change compared to the Jaccard similarity of entity content illustrated in \figref{ch_temporal_el:fig:evolution_entities_jaccard}. This suggests that the context around the anchor mentions 
%tends to undergo%
undergoes
a higher degree of temporal 
% change 
% drift
transformation
compared to that of target entities. 
% We leave for future work a more detailed analysis on tracing the evolution of the context around each of the individual mentions, as well as on the creation of new mentions linked to specific entity.
% \revklim{TODO: please put here ideas for statistics!!} 
% \lucie{I think it would be nice here to get a few things that change over time, to focus on how much this impacts performance}
% \revklim{
% \begin{enumerate}
%     \item Graph with sizes of different categories (random, new entities) per subset.
%     \item Graph of mentions per entity $\rightarrow$ how?
%     \item (related to previous one) Graph of nr of inlinks vs the number of distinct mentions in order to show how diverse the dataset is.?
%     \lucie{\item Something about how context of mentions changes}
%     \begin{itemize}
%         \item WIP: see \figref{fig:evolution_mentions}, still missing dot product of representations. 
%     \end{itemize}
%     \lucie{\item Something about how the entity page changes over time}
%     \begin{itemize}
%         \item WIP: see \figref{fig:evolution_entities}, still missing dot product of representations. 
%     \end{itemize}
% \end{enumerate}
% }
% BEGIN we are here 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Script to generate these graphs: 
% https://gitlab.ilabt.imec.be/kzaporoj/el_copenhagen/-/blob/main/src/wiki/wikipedia/jobs/dataset_creation/s06_final_dataset_statistics_change.py
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{figure}[!t]
% \centering
% \includegraphics[width=0.8\columnwidth, trim={0.0cm 0.0cm 0.0cm 0.0cm},clip]{jackard_entities_years.pdf}
% \caption{Change entity description in time (fixed nr of tokens across years). Edit distance is normalized between 0 and 1. }
% \label{ch_temporal_el:fig:evolution_entities}
% \end{figure}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% % Script to generate these graphs: 
% % https://gitlab.ilabt.imec.be/kzaporoj/el_copenhagen/-/blob/main/src/wiki/wikipedia/jobs/dataset_creation/s06_final_dataset_statistics_change.py
% csv located at: 
% https://cloud.ilabt.imec.be/index.php/s/NEx7egfiMGweAbX
% script for all the graphs (input are the csv files): 
% src/wiki/wikipedia/jobs/stats/s08_all_paper_stats.py
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[t]
\begin{subfigure}{.31\textwidth}
  \centering
  % include first image
  \includegraphics[width=1.0\linewidth]{s08_jaccard_entities_change.pdf}  
  % \caption{Jaccard vocabulary similarity between entity content in 2013 and the next years.}
  \caption{Evolution of entities in terms of Jaccard vocabulary similarity.}
  \label{ch_temporal_el:fig:evolution_entities_jaccard}
\end{subfigure} \hfill
\begin{subfigure}{.31\textwidth}
  \centering
  % include second image
  \includegraphics[width=1.0\linewidth]{s08_edit_distance_entities_change.pdf}  
  \caption{Evolution of entities in terms of edit distance of the content.}
  \label{ch_temporal_el:fig:evolution_entities_edistance}
\end{subfigure} \hfill
% \begin{subfigure}{.66\textwidth}
%   \centering
%   % include second image
%   \includegraphics[width=1.0\linewidth]{jackard_entities_years_v3.pdf}  
%   \caption{}
%   \label{ch_temporal_el:fig:evolution_entities_edistance}
% \end{subfigure}
\begin{subfigure}{.31\textwidth}
  \centering
  % include second image
  \includegraphics[width=1.0\linewidth]{s08_jaccard_mentions_change.pdf}  
  \caption{Evolution of context around the mentions (Jaccard similarity).}
  \label{ch_temporal_el:fig:evolution_mentions}
\end{subfigure}
\caption{Change of textual content of entities and context around mentions across temporal yearly cuts (x-axis). }
% \caption[test]{Change entity description in time (fixed nr of tokens across years). Edit distance is normalized between 0 and 1.}
\label{ch_temporal_el:fig:fig}
\end{figure}


% \begin{figure}[!t]
% \centering
% \includegraphics[width=0.5\columnwidth, trim={0.0cm 0.0cm 0.0cm 0.0cm},clip]{jackard_mentions_years_v3.pdf}
% \caption{Change mention context in time (fixed nr of tokens across years). First drop makes sense since we do not track each of the mentions individually (as is the case of entity text), the mentions are picked more or less randomly for each of the cuts. }
% \label{ch_temporal_el:fig:evolution_mentions}
% \end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Script to generate these graph: 
% https://gitlab.ilabt.imec.be/kzaporoj/el_copenhagen/-/blob/main/src/wiki/wikipedia/jobs/dataset_creation/s04_final_dataset_statistics.py
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{figure}[!t]
% \centering
% \includegraphics[width=1.0\columnwidth, trim={0.0cm 0.0cm 0.0cm 0.0cm},clip]{train_mentions_per_entity.pdf}
% \caption{Distribution of the data across the cuts (should be the same, but it is not for new entities, working to fix this and the variation in \tabref{tab:dataset_detail}!). }
% \label{ch_temporal_el:fig:men_entity_distribution}
% \end{figure}



% \subsection{Dataset construction}

% \subsubsection{Dataset split}
% Each of the temporal snapshots is divided into train, 
% validation and test subsets. See table \tabref{tab:dataset} for additional stats. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Script to generate this table: 
% https://gitlab.ilabt.imec.be/kzaporoj/el_copenhagen/-/blob/main/src/wiki/wikipedia/jobs/dataset_creation/s04_final_dataset_statistics.py
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[t]
\centering
% \resizebox{0.55\columnwidth}{!}
% {
\caption{Summarized statistics of \ourdataset.}
\label{ch_temporal_el:tab:dataset_detail2}
\begin{tabular}{l ccc}
        \toprule
         Statistic & \multicolumn{1}{c}{Train} & \multicolumn{1}{c}{Validation} & \multicolumn{1}{c}{Test} \\ 
         \midrule 
         Temporal Snapshots & 10 & 10 & 10 \\ % \vspace{0.05 in}\\
        %  \midrule
         Shared Entities & 10,000 & 10,000 & 10,000 \\
         \ \ \ \# Anchor Mentions & 223,436 & 77,148 & 72,012 \\ % \vspace{0.05 in} \\
        %  \midrule
        %  \ \ \ Avg. Target Length (tokens) & ? & ? & ? \\
        %  \ \ \ Avg. Anchor Length (tokens) & ? & ? & ? \vspace{0.05 in}\\ 
        %  New Entities & \multicolumn{3}{c}{431} \\
        New Entities & 431 & 431 & 431 \\
         \ \ \ \# Anchor Mentions & 1,873 & 2,636 & 2,190 \\
        %  \ \ \ Avg. Target Length (tokens) & ? & ? & ? \\
        %  \ \ \ Avg. Anchor Length (tokens) & ? & ? & ? \\
        \bottomrule % \vspace{-0.08 in}
        \end{tabular}
        % }
\end{table}
% \begin{table}[t]
% \centering
% \resizebox{1.0\columnwidth}{!}
% {\begin{tabular}{l cc c ccc c ccc}
%         \toprule
%          & \multicolumn{2}{c}{\#Entities} && \multicolumn{3}{c}{\#Mentions Shared} && \multicolumn{3}{c}{\#Mentions New} \\ 
%         \cmidrule(lr){2-3}\cmidrule(lr){5-7}\cmidrule(lr){9-11}
%         Cut & \ Shared & \ New && \# Train & \# Validation & \# Test && \# Train & \# Validation & \# Test \\ 
%         \midrule
%                 2013 & 15000 & 431 && 223436 & 77148 & 72012 && 1873 & 2636 & 2190 \\ 
%                 2014 & 15000 & 431 && 223437 & 77147 & 72012 && 1873 & 2636 & 2190 \\ 
%                 2015 & 15000 & 431 && 223442 & 77149 & 72012 && 1873 & 2636 & 2190 \\ 
%                 2016 & 15000 & 431 && 223442 & 77148 & 72012 && 1873 & 2636 & 2190 \\ 
%                 2017 & 15000 & 431 && 223442 & 77149 & 72012 && 1873 & 2636 & 2190 \\ 
%                 2018 & 15000 & 431 && 223442 & 77149 & 72011 && 1873 & 2636 & 2190 \\ 
%                 2019 & 15000 & 431 && 223442 & 77148 & 72011 && 1873 & 2636 & 2190 \\ 
%                 2020 & 15000 & 431 && 223440 & 77148 & 72011 && 1872 & 2636 & 2190 \\ 
%                 2021 & 15000 & 431 && 223441 & 77147 & 72013 && 1873 & 2636 & 2190 \\ 
%                 2022 & 15000 & 431 && 223442 & 77147 & 72012 && 1873 & 2636 & 2190 \\ 
%         \bottomrule
%         \end{tabular}}
%         \caption{Distribution across subsets.}
%         \label{ch_temporal_el:tab:dataset_detail2}
% \end{table}
% \begin{table}[t]
%     \centering
%     \resizebox{0.7\columnwidth}{!}
%     {\begin{tabular}{l c c c c c}
%         \toprule
%           & \# Shared & \# New & \multicolumn{1}{c}{Train} & \multicolumn{1}{c}{Validation} & \multicolumn{1}{c}{Test} \\
%         %   \cmidrule(lr){3-3}\cmidrule(lr){5-5}\cmidrule(lr){7-7}
%           Cut & Entities & Entities & \# Mentions & \# Mentions & \# Mentions \\
%          \midrule
%         2013 & ? & ? & ? & ? & ? \\ 
% 	 \bottomrule
%     \end{tabular}}
%     \caption{Distribution across subsets.} 
%     \label{ch_temporal_el:tab:dataset}
% \end{table}
% \begin{table}[t]
%     \centering
%     \resizebox{1.0\columnwidth}{!}
%     {\begin{tabular}{l cc c cc c cc}
%         \toprule
%           & \multicolumn{2}{c}{Train} && \multicolumn{2}{c}{Validation} && \multicolumn{2}{c}{Test} \\
%           \cmidrule(lr){2-3}\cmidrule(lr){5-6}\cmidrule(lr){8-9}
%           Cut & \# Entities & \# Mentions && \# Entities & \# Mentions && \# Entities & \# Mentions \\
%          \midrule
%         2013 & 11634 & 71250 && 11634 & 42671 && 11634 & 40426 \\ 
%         2014 & 11615 & 70635 && 11615 & 42044 && 11615 & 40572 \\ 
%         2015 & 11664 & 70707 && 11664 & 42642 && 11664 & 40392 \\ 
%         2016 & 11735 & 69661 && 11735 & 42687 && 11735 & 40468 \\ 
%         2017 & 11716 & 71120 && 11716 & 41835 && 11716 & 40331 \\ 
%         2018 & 11648 & 70929 && 11648 & 41864 && 11648 & 40887 \\ 
%         2019 & 11633 & 69950 && 11633 & 42323 && 11633 & 40537 \\ 
%         2020 & 11697 & 70711 && 11697 & 42117 && 11697 & 40939 \\ 
%         2021 & 11827 & 72986 && 11827 & 42176 && 11827 & 41171 \\ 
%         2022 & 11912 & 71189 && 11912 & 42311 && 11912 & 40918 \\ 
% 	 \bottomrule
%     \end{tabular}}
%     \caption{Distribution across subsets.} 
%     \label{ch_temporal_el:tab:dataset}
% \end{table}
\section{Experiments}
% We follow the evaluation setup used in recent work on temporal evolution . 
We divide our dataset in 10 different yearly snapshots and evaluate on each of them individually. This evaluation setup allows us to measure the change in model performance over time, revealing the degree in which each of the temporal periods are affected \cite{agarwal2021temporal, he2018time, luu2021time}. 
% For training, we recognise two possible scenarios. 
We train on each of the temporal snapshots separately and evaluate on all of the past and future time periods. 

Our experiments are directed to answer the following research questions:~\begin{enumerate*}[label=\textbf{(Q\arabic*)}]
    \item \label{ch_temporal_el:it:q1-temp-degradation} Is there a general temporal degradation in performance?
    \item \label{ch_temporal_el:it:q2-fine-tuning} Does fine-tuning help improve the performance for a particular temporal snapshot compared to past and future snapshots?
    \item \label{ch_temporal_el:it:q3-emerging} How the performance of \textit{new} emerging entities in each of the temporal snapshots compares to that of \textit{shared} entities?
\end{enumerate*}
% This approach is also adopted in recent related work REF and contrasts with accumulative approach where the model is continuously fed new time snapshots, which we leave for future work. 
% This method used in REF has the advantage of ... \revklim{TODO}. 
% The second method consists in using some sort of continual learning technique (REF). We leave it for the future work. 

% An alternative evaluation scenario would .... While the structure of our dataset supports this evaluation approach
% \revklim{Somehow tie it with the setup of \cite{agarwal2021temporal,huang2018examining}, also in \cite{lazaridou2021mind,rottger2021temporal}. Might be also interesting to look in the past by testing on previous years...}. This contrasts with evolutionary setup proposed used... continual learning can be used... We leave continual modelling setup for the future work. 

% Therefore, we decided to follow related work in \cite{agarwal2021temporal, loureiro2022timelms}, and only fine-tune our models on the available task-dependent training set data for each of the temporal cuts. 



% \begin{enumerate}
%     \item 
%     \item 
% \end{enumerate}
\subsection{Baseline}
We experiment with the bi-encoder \cite{mazare2018training,dinan2018wizard} baseline introduced in BLINK model proposed by \cite{wu2019zero}. This method encodes independently the mention contexts as well as the entity descriptions and then performs the retrieval in a dense space \cite{karpukhin2020dense} by matching the context of each mention with the closest candidate entities.  
% Following this method, we fine-tune the bi-encoder \cite{mazare2018training,dinan2018wizard} on ... \revklim{we are here}
% bi-encoder == DPR?? 
Similarly to \cite{agarwal2021temporal, loureiro2022timelms}, we experiment only with fine-tuning of our BERT based model. We leave a complete pre-training on each of the Wikipedia snapshots for future work. 
% Similarly to \cite{agarwal2021temporal, loureiro2022timelms}, in this work we experiment with fine-tuning of our BERT-based model only. 
% Due to the limitation in the resources, we leave the study of the impact of complete pre-training of the BERT model on yearly Wikipedia snapshots for future work. 
% snapshots would require substantially more computational resources.
% of the  follow the trend of recent work  and focus only on evaluating the fine-tuning effect on our BERT-based model \cite{wu2019zero}. 
% A complete pre-training of the BERT on the yearly Wikipedia snapshots would require substantially more computational resources. 
% \textit{fine-tuning} and not \textit{pre-training} since pre-training require substantially more computational resources. Other previous work \cite{agarwal2021temporal, rottger2021temporal} have also used already pre-trained models and only fine-tuned to study temporal effects. 
% In order to reveal the effect of fine-tuning we use shared target entities across the different years (the ones that model would have ``seen'' during fine-tuning) together with new unseen (emerging) entities that appear in each of the temporal snapshots (see \figref{fig:el_introduction} for example and \tabref{tab:dataset} for stats). 
% \begin{enumerate}
%     \item One baseline involving Wikipedia only \cite{wu2019zero}
%     \item One baseline involving Wikipedia+Wikidata \cite{orr2020bootleg}
% \end{enumerate}
% A table like in figure 4 of \url{https://datasets-benchmarks-proceedings.neurips.cc/paper/2021/file/4c56ff4ce4aaf9573aa5dff913df997a-Paper-round1.pdf} would be nice. 
\subsection{Results and Analysis}
\label{ch_temporal_el:sec:results_and_analysis}
%%%%%%%%%%%%%%%%%%%%
% code to generate results for this stats: 
% https://gitlab.ilabt.imec.be/kzaporoj/el_copenhagen/-/blob/main/src/wiki/wikipedia/jobs/models/s07_analyze_similarity_of_predicted_candidates.py
% csv file inside https://cloud.ilabt.imec.be/index.php/s/NEx7egfiMGweAbX     (candidate_similarity_jaccard.csv)
%%%%%%%%%%%%%%%%%%%%
% \begin{figure}[!t]
% \centering
% \includegraphics[width=0.35\columnwidth, trim={0.0cm 0.0cm 0.0cm 0.0cm},clip]{s08_candidate_similarity_jaccard.pdf}
% \caption{Jaccard Similarity between top 64 candidate entities extracted by fine-tuned bi-encoders across the years.}
% \label{ch_temporal_el:fig:el_pipeline}
% \end{figure}
\begin{figure}[t]
% \centering
\begin{subfigure}{.32\textwidth}
  \centering
  % include first image
  \includegraphics[width=1.0\linewidth]{s08_candidate_similarity_jaccard.pdf}  
  \caption{Similarity between candidates returned by the bi-encoder baseline.}
  \label{ch_temporal_el:fig:candidate_similarity}
\end{subfigure}\hfill
\begin{subfigure}{.32\textwidth}
  \centering
  % include second image
  \includegraphics[width=1.0\linewidth]{s08_results_new_vs_shared.pdf}  
  \caption{Difference in performance between \textit{new} and \textit{shared} entities.}
  \label{ch_temporal_el:fig:avg_performance}
\end{subfigure}\hfill
\begin{subfigure}{.32\textwidth}
  \centering
  % include second image
  \includegraphics[width=1.0\linewidth]{s08_nr_wiki_candidates.pdf}  
  \caption{Evolution of the number of entities in the Wikipedia KB.}
  \label{ch_temporal_el:fig:nr_wiki_entities}
\end{subfigure}
% \caption{Jaccard Similarity between top 64 candidate entities extracted by fine-tuned bi-encoders across the years. Also average performance between new and shared entities.}
\caption{Statistics related to the analysis of the results (\secref{ch_temporal_el:sec:results_and_analysis}) across the temporal cuts (x-axis).}
\label{ch_temporal_el:fig:candidates_and_performance}
\end{figure}
% \begin{figure}[ht]
% \begin{subfigure}{0.5\textwidth}
%   \centering
%   % include second image
%   \includegraphics[width=1.0\linewidth]{jaccard_similarity_between_candidates.pdf}  
%   \caption{}
%   \label{ch_temporal_el:fig:cand_jaccard_similarity}
% \end{subfigure}
% \caption{Jaccard similarity between top 64 candidate entities extracted by fine-tuned bi-encoders across the years.}
% \label{ch_temporal_el:fig:fig_similarity_candidates}
% \end{figure}

% In the results, we see that there are still significant challenges for temporal entity linking, making this dataset an important contribution. In particular, we find that entity linking to entities not seen in training decrease performance significantly. However, this is a setup that comes close to real-world challenges, where entity linking tools need to cope with the ever-changing nature of the world and its mentions. In the following, we describe the results for both setups, with shared and new entities respectively and their implications.
%
% \subsubsection{Shared entities}
% Shared entities are entities that exist throughout the years. We use them as a proxy to understand change in context and how entity linking models cope with this change in context of a mention as well as the candidate entity itself.
The results for \textit{shared} and \textit{new} entities are shown in \tabref{ch_temporal_el:tab:general_table_shared}.
% and \tabref{tab:general_table_new_entities} respectively. 
The used metric is Accuracy@64 which,  for each of the anchor mentions, assigns positive score if any of the top 64 candidate entities returned by the bi-encoder is correct. 
We observe a consistent temporal decrease in performance for \textit{shared} entities (\ref{ch_temporal_el:it:q1-temp-degradation}). This is also observed in \figref{ch_temporal_el:fig:avg_performance}, which showcases the average temporal degradation across all the fine-tuned models. 
We hypothesise that one of the reasons of 
this temporal degradation in performance is the temporal increase in the number of more similar (\ie granular) entities. In order to demonstrate this, we calculate the \textit{Jaccard Similarity} between consecutive descriptions of top 64 candidate entities returned by the bi-encoder. We observe a consistent increase in this similarity metric illustrated in \figref{ch_temporal_el:fig:candidate_similarity}. This growth in more similar entities is accompanied with a general increase in the number of entities in the Wikipedia KB (see \figref{ch_temporal_el:fig:nr_wiki_entities}). As a consequence, the model is given an ever-increasing number of candidate target entities, which can potentially impact its performance.

Furthermore, we observe a limited effect of fine-tuning on both \textit{shared} as well as \textit{new} entities, with only a slight improvement for some of the snapshots \ref{ch_temporal_el:it:q2-fine-tuning}. This is consistent with findings in previous work on temporal degradation for different tasks \cite{agarwal2021temporal} using Transformer \cite{vaswani2017attention} based models, where the authors observe that original pre-trained representations are extremely expressive, often outweighing the effect of fine-tuning on downstream tasks.  
% and often outweigh the effect of fine-tuning to incorporate additional evolutionary knowledge in the model. 
% often contain contain enough information .... 
% \revklim{TODO}....  
Yet, following this logic we do not observe a major decrease in performance after 2018, which is the year the original Transformer based BERT \cite{devlin2019bert} model was pre-trained (see \figref{ch_temporal_el:fig:avg_performance}). This leads us to hypothesise that the actual knowledge needed to disambiguate most of the entities in \ourdataset~changes very little with time. In order to prove this for \textit{shared}\footnote{We analyze the same effect on \textit{new} entities in the next paragraph.} entities, we manually analyzed the difference in mention contexts and entity contents of random 100 
entity-mentions pairs
% most dissimilar (Jaccard Similarity) 
% entities 
between the years 2013 and 2022. We found that in most of the cases (above 95\%), while the textual description of the shared entity is changed (supported by \figsref{ch_temporal_el:fig:evolution_entities_jaccard}{ch_temporal_el:fig:evolution_entities_edistance}), its meaning remains the same. This suggests that the knowledge present in the original pre-trained BERT is sufficient to also be applied to more recent versions of existing 
% mentions and entities 
entities
in Wikipedia.  % \ref{ch_temporal_el:it:q2-fine-tuning}
% This explains why models fine-tuned and tested on a specific snapshot perform on par with other models fine-tuned on different snapshots

% P3 goal: fine-tuning little effect; new entities not the same as new knowledge; no big drop after bert 2018 pre-trained
Finally, we analyze the performance on \textit{new} entities and how it compares to the performance on \textit{shared} entities \ref{ch_temporal_el:it:q3-emerging}. 
We plot the average temporal change in Accuracy@64 score across all fine-tuned models for both types of entities in \figref{ch_temporal_el:fig:avg_performance}.
% We were surprised by relatively little difference in Acc@64 scores (even slightly better performance for years 2013 and 2014) compared to \textit{shared} entities. 
We observe that, in general, the performance on \textit{shared} entities is superior to that on \textit{new} entities. However, this difference is relatively small, with high variation between different temporal snapshots (\eg increase between the years 2013 and 2014 and decrease for the snapshot taken at the end of 2020). 
In order to understand this behaviour, we manually analyze 100 random new entities from our dataset. We found that the big majority of entities (around 90\% of cases) were either extracts of already existing pages or events that are repetitive in nature (\eg ``2018 BNP Paribas Open''). We conjecture that these entities require little additional knowledge to be disambiguated, since either they already exist (as part of the content of other entities) or are very similar to already existing entities in Wikipedia. 
This is supported by the lower performance on the temporal snapshot 2021 driven mostly by COVID-19 related entities, which constitute 19\% of entities linked to by 56\% of mentions. The disambiguation of these cases requires a completely new and 
% radically 
fundamentally
different, previously non-existent knowledge. This knowledge is not present in the original corpus used to pre-train BERT model, posing a challenge to the BERT based bi-encoder baseline. In fact, our further analysis showcases a difference in performance of more than 22\% Accuracy@64 points on such cases compared to the rest of the mentions linked to \textit{new} entities.\footnote{0.4265 for COVID-related new entities and 0.6510 for the rest of the new entities.}
% \tabref{ch_temporal_el:tab:covid_vs_non_covid} showcases a difference in performance of more than 22\% Accuracy@64 points on such cases compared to the rest of the mentions linked to \textit{new} entities. 
%\revklim{No fine-tuning effect due to small size of new covid-related mentions compared to shared ones?}
% This is explained by the fact that COVID related entities are completely new and require additional knowledge not present in the originally pre-trained BERT model. 
%These entities are completely new and require additional knowledge not present in the original pre-trained BERT model. 
% We further zoom in the snapshot 2021 and discover that it has a higher proportion of new entities related to COVID-19 pandemic (19\% of entities which are linked to by 56\% of mentions). \Tabref{ch_temporal_el:tab:covid_vs_non_covid} showcases a difference in performance of more than 22\% Acc@64 points on COVID related cases. 
% We hypothesise that pre-trained BERT model lacks the
% in 31\% the new entities were actually extracts of already existing Wikipedia pages... 
% Furthermore, 59\%  of mentions pointed to new entities referring to frequently occurring events such as \revklim{League...} . Finally, only x\% of entities were considered as completely new without any historic precedent in the last 10 years. 
% We further analyze the year 2021 were there is a significant decrease in performance for \textit{new} entities in Wikipedia. 
% We discover that this year presents an increase of entities requiring completely new knowledge regarding the pandemic COVID-19 (eg...).  The exception was the proportion changed t
% and y\% of new entities ... Furthermore, in z\% of new entities
% As a consequence, we speculate that the model has 
% \revklim{\begin{enumerate}
%     \item consistent decrease for shared
%     \item fine-tuning of no effect
% \end{enumerate}}


%
% In Table~\ref{ch_temporal_el:tab:general_table_shared} are the results for the models fine-tuned on the datasets (column) and their performance over the test datasets of different years (row). Performance for each of the entity linking models decreases over time. While this is to be expected we make the following additional observations; the models performance \textit{increases} for previous years; the model fine-tuned on the data of 2013 performs best over all years.
%
% We attribute these phenomena to the following attributes: The models perform well on previous years as the content of the target entity is not removed and replaced, but in Wikipedia typically articles grow in content, keeping older information alongside the new information \cite{aaltonen2016cumulative}. This could explain why the models perform well on past instances of Wikipedia.
%
% Since we only regard entities that are shared in this setup, i.e., have existed since 2013, it is to consider that those entities are usually less fine-grained than the entities introduced later, i.e., Wikipedia pages on complex topics are split into multiple pages later, leading to a larger number of entities, which are similar.
%
% Lastly, it is to assume the 2013 model performs better, as it has less entities to disambiguate against. Since here, it has seen all entities in the fine-tuning, there is a higher chance of the 2013 model to pick the right candidates purely on the limited number of candidates it selects from.

% \subsubsection{New Entities}
%
% Overall, there is still a trend of the performance decreasing for new entities in the future. However, trends are not as clear, as new entities can change quite dramatically between the years; e.g., how similar they are to existing entities, making it easier or harder to link the mentions to the candidates. This could explain, for example, why all models drop in performance on the data of 2021.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Script to generate the result tables: 
% src/wiki/wikipedia/jobs/models/s07_calculate_results_and_metrics_blink.py
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[t] 
\caption{Accuracy@64 for \textit{shared} (top) and \textit{new} (bottom) entities. The intensity of colours is organized by row and represents \textcolor{darkspringgreen!100}{\textbf{higher}} and \textcolor{deepcarmine!100}{\textbf{lower}} results with respect to the year the model was fine-tuned on. The best values for each column are \underline{underlined}.} 
        \label{ch_temporal_el:tab:general_table_shared}
\centering 
\resizebox{0.9\columnwidth}{!} {
\begin{tabular}{c cccccccccc} 
         \toprule
         \multicolumn{11}{c}{Shared Entities} \\
         \midrule
         \textbf{Models} & 2013 & 2014 & 2015 & 2016 & 2017 & 2018 & 2019 & 2020 & 2021 & 2022 \\ 
        \midrule 
% 2013  & 0.726 & \cellcolor{deepcarmine!17}0.721 & \cellcolor{deepcarmine!18}0.720 & \cellcolor{deepcarmine!31}0.712 & \cellcolor{deepcarmine!42}0.705 & \cellcolor{deepcarmine!46}0.702 & \cellcolor{deepcarmine!52}0.699 & \cellcolor{deepcarmine!61}0.692 & \cellcolor{deepcarmine!63}0.691 & \cellcolor{deepcarmine!75}0.684 \\ 
2014  & \cellcolor{darkspringgreen!17}0.692 & 0.687 & \cellcolor{deepcarmine!14}0.684 & \cellcolor{deepcarmine!27}0.676 & \cellcolor{deepcarmine!41}0.666 & \cellcolor{deepcarmine!39}0.668 & \cellcolor{deepcarmine!50}0.661 & \cellcolor{deepcarmine!62}0.653 & \cellcolor{deepcarmine!63}0.652 & \cellcolor{deepcarmine!75}0.645 \\ 
2015  & \cellcolor{darkspringgreen!20}0.683 & \cellcolor{darkspringgreen!12}0.678 & 0.677 & \cellcolor{deepcarmine!24}0.668 & \cellcolor{deepcarmine!40}0.658 & \cellcolor{deepcarmine!36}0.660 & \cellcolor{deepcarmine!49}0.652 & \cellcolor{deepcarmine!60}0.645 & \cellcolor{deepcarmine!62}0.644 & \cellcolor{deepcarmine!75}0.636 \\ 
2016  & \cellcolor{darkspringgreen!44}\underline{0.706} & \cellcolor{darkspringgreen!31}\underline{0.700} & \cellcolor{darkspringgreen!26}\underline{0.697} & \underline{0.689} & \cellcolor{deepcarmine!28}\underline{0.680} & \cellcolor{deepcarmine!27}\underline{0.681} & \cellcolor{deepcarmine!37}\underline{0.676} & \cellcolor{deepcarmine!55}\underline{0.667} & \cellcolor{deepcarmine!61}\underline{0.665} & \cellcolor{deepcarmine!75}\underline{0.658} \\ 
2017  & \cellcolor{darkspringgreen!73}0.688 & \cellcolor{darkspringgreen!58}0.683 & \cellcolor{darkspringgreen!51}0.680 & \cellcolor{darkspringgreen!32}0.673 & 0.665 & \cellcolor{deepcarmine!12}0.664 & \cellcolor{deepcarmine!33}0.657 & \cellcolor{deepcarmine!55}0.649 & \cellcolor{deepcarmine!59}0.647 & \cellcolor{deepcarmine!75}0.642 \\ 
2018  & \cellcolor{darkspringgreen!75}0.692 & \cellcolor{darkspringgreen!58}0.686 & \cellcolor{darkspringgreen!50}0.683 & \cellcolor{darkspringgreen!30}0.676 & \cellcolor{deepcarmine!15}0.667 & 0.669 & \cellcolor{deepcarmine!29}0.662 & \cellcolor{deepcarmine!53}0.653 & \cellcolor{deepcarmine!59}0.651 & \cellcolor{deepcarmine!74}0.646 \\ 
2019  & \cellcolor{darkspringgreen!75}0.693 & \cellcolor{darkspringgreen!63}0.688 & \cellcolor{darkspringgreen!61}0.687 & \cellcolor{darkspringgreen!42}0.678 & \cellcolor{darkspringgreen!23}0.670 & \cellcolor{darkspringgreen!23}0.669 & 0.663 & \cellcolor{deepcarmine!31}0.653 & \cellcolor{deepcarmine!32}0.653 & \cellcolor{deepcarmine!47}0.646 \\ 
2020  & \cellcolor{darkspringgreen!75}0.701 & \cellcolor{darkspringgreen!65}0.695 & \cellcolor{darkspringgreen!62}0.693 & \cellcolor{darkspringgreen!48}0.685 & \cellcolor{darkspringgreen!32}0.676 & \cellcolor{darkspringgreen!35}0.678 & \cellcolor{darkspringgreen!21}0.670 & 0.663 & \cellcolor{deepcarmine!13}0.661 & \cellcolor{deepcarmine!26}0.654 \\ 
2021  & \cellcolor{darkspringgreen!75}0.696 & \cellcolor{darkspringgreen!66}0.690 & \cellcolor{darkspringgreen!62}0.688 & \cellcolor{darkspringgreen!51}0.681 & \cellcolor{darkspringgreen!35}0.672 & \cellcolor{darkspringgreen!37}0.673 & \cellcolor{darkspringgreen!29}0.668 & \cellcolor{darkspringgreen!15}0.659 & 0.656 & \cellcolor{deepcarmine!19}0.650 \\ 
2022  & \cellcolor{darkspringgreen!75}0.703 & \cellcolor{darkspringgreen!66}0.697 & \cellcolor{darkspringgreen!63}0.695 & \cellcolor{darkspringgreen!53}0.688 & \cellcolor{darkspringgreen!40}0.678 & \cellcolor{darkspringgreen!41}0.678 & \cellcolor{darkspringgreen!33}0.673 & \cellcolor{darkspringgreen!21}0.664 & \cellcolor{darkspringgreen!18}0.662 & 0.656 \\ 
        \midrule
        % \vspace{0.01}
        \multicolumn{11}{c}{New Entities} \\
         \midrule 
         \textbf{Models} & 2013 & 2014 & 2015 & 2016 & 2017 & 2018 & 2019 & 2020 & 2021 & 2022 \\ 
        \midrule 
% 2013  & 0.748 & \cellcolor{darkspringgreen!14}0.760 & \cellcolor{deepcarmine!19}0.726 & \cellcolor{deepcarmine!19}0.726 & \cellcolor{deepcarmine!38}0.680 & \cellcolor{deepcarmine!38}0.679 & \cellcolor{deepcarmine!45}0.662 & \cellcolor{deepcarmine!35}0.687 & \cellcolor{deepcarmine!75}0.590 & \cellcolor{deepcarmine!49}0.653 \\ 
2014  & \cellcolor{darkspringgreen!13}0.700 & 0.692 & \cellcolor{deepcarmine!21}0.663 & \cellcolor{deepcarmine!48}0.597 & \cellcolor{deepcarmine!45}0.602 & \cellcolor{deepcarmine!44}0.607 & \cellcolor{deepcarmine!46}0.601 & \cellcolor{deepcarmine!50}0.589 & \cellcolor{deepcarmine!75}0.529 & \cellcolor{deepcarmine!39}0.618 \\ 
2015  & \cellcolor{darkspringgreen!37}0.690 & \cellcolor{darkspringgreen!25}0.672 & 0.648 & \cellcolor{deepcarmine!48}0.589 & \cellcolor{deepcarmine!42}0.597 & \cellcolor{deepcarmine!48}0.589 & \cellcolor{deepcarmine!44}0.595 & \cellcolor{deepcarmine!38}0.604 & \cellcolor{deepcarmine!75}0.548 & \cellcolor{deepcarmine!35}0.609 \\ 
2016  & \cellcolor{darkspringgreen!60}\underline{0.717} & \cellcolor{darkspringgreen!67}\underline{0.725} & \cellcolor{darkspringgreen!29}0.677 & \underline{0.652} & \cellcolor{deepcarmine!12}\underline{0.649} & \cellcolor{deepcarmine!27}0.630 & \cellcolor{deepcarmine!38}0.616 & \cellcolor{deepcarmine!21}0.637 & \cellcolor{deepcarmine!75}0.569 & \cellcolor{deepcarmine!24}0.634 \\ 
2017  & \cellcolor{darkspringgreen!75}0.705 & \cellcolor{darkspringgreen!73}0.703 & \cellcolor{darkspringgreen!49}0.670 & \cellcolor{darkspringgreen!13}0.621 & 0.616 & \cellcolor{deepcarmine!17}0.606 & \cellcolor{deepcarmine!26}0.594 & \cellcolor{deepcarmine!17}0.606 & \cellcolor{deepcarmine!66}0.539 & \cellcolor{deepcarmine!12}0.613 \\ 
2018  & \cellcolor{darkspringgreen!75}0.693 & \cellcolor{darkspringgreen!68}0.685 & \cellcolor{darkspringgreen!48}0.658 & \cellcolor{deepcarmine!12}0.604 & \cellcolor{deepcarmine!11}0.605 & 0.607 & \cellcolor{deepcarmine!21}0.592 & \cellcolor{deepcarmine!19}0.595 & \cellcolor{deepcarmine!52}0.551 & \cellcolor{darkspringgreen!17}0.618 \\ 
2019  & \cellcolor{darkspringgreen!74}0.701 & \cellcolor{darkspringgreen!75}0.702 & \cellcolor{darkspringgreen!54}0.670 & \cellcolor{deepcarmine!10}0.603 & \cellcolor{darkspringgreen!19}0.618 & \cellcolor{darkspringgreen!12}0.607 & 0.603 & \cellcolor{deepcarmine!14}0.596 & \cellcolor{deepcarmine!59}0.527 & \cellcolor{darkspringgreen!13}0.608 \\ 
2020  & \cellcolor{darkspringgreen!70}0.716 & \cellcolor{darkspringgreen!75}0.722 & \cellcolor{darkspringgreen!54}\underline{0.695} & \cellcolor{darkspringgreen!10}0.635 & \cellcolor{darkspringgreen!10}0.635 & \cellcolor{deepcarmine!11}\underline{0.633} & \cellcolor{deepcarmine!18}\underline{0.624} & 0.635 & \cellcolor{deepcarmine!62}0.565 & \cellcolor{deepcarmine!16}0.627 \\ 
2021  & \cellcolor{darkspringgreen!75}0.705 & \cellcolor{darkspringgreen!72}0.698 & \cellcolor{darkspringgreen!57}0.664 & \cellcolor{darkspringgreen!34}0.609 & \cellcolor{darkspringgreen!39}0.622 & \cellcolor{darkspringgreen!34}0.609 & \cellcolor{darkspringgreen!30}0.600 & \cellcolor{darkspringgreen!41}0.625 & 0.552 & \cellcolor{darkspringgreen!49}\underline{0.645} \\ 
2022  & \cellcolor{darkspringgreen!75}0.716 & \cellcolor{darkspringgreen!71}0.712 & \cellcolor{darkspringgreen!47}0.685 & \cellcolor{deepcarmine!12}0.639 & \cellcolor{deepcarmine!12}0.639 & \cellcolor{deepcarmine!17}\underline{0.633} & \cellcolor{deepcarmine!27}0.622 & \cellcolor{deepcarmine!12}\underline{0.639} & \cellcolor{deepcarmine!72}\underline{0.570} & 0.642 \\ 
        \bottomrule         
        \end{tabular}}
        % } 
\end{table}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Script to generate the result tables: 
% src/wiki/wikipedia/jobs/models/s07_calculate_results_and_metrics_blink.py
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{table}[t] 
% \centering 
% \resizebox{0.9\columnwidth}{!} 
% {\begin{tabular}{c cccccccccc} 
%          \toprule 
%          \textbf{Models} & 2013 & 2014 & 2015 & 2016 & 2017 & 2018 & 2019 & 2020 & 2021 & 2022 \\ 
%         \midrule 
% % 2013  & 0.748 & \cellcolor{darkspringgreen!14}0.760 & \cellcolor{deepcarmine!19}0.726 & \cellcolor{deepcarmine!19}0.726 & \cellcolor{deepcarmine!38}0.680 & \cellcolor{deepcarmine!38}0.679 & \cellcolor{deepcarmine!45}0.662 & \cellcolor{deepcarmine!35}0.687 & \cellcolor{deepcarmine!75}0.590 & \cellcolor{deepcarmine!49}0.653 \\ 
% 2014  & \cellcolor{darkspringgreen!13}0.700 & 0.692 & \cellcolor{deepcarmine!21}0.663 & \cellcolor{deepcarmine!48}0.597 & \cellcolor{deepcarmine!45}0.602 & \cellcolor{deepcarmine!44}0.607 & \cellcolor{deepcarmine!46}0.601 & \cellcolor{deepcarmine!50}0.589 & \cellcolor{deepcarmine!75}0.529 & \cellcolor{deepcarmine!39}0.618 \\ 
% 2015  & \cellcolor{darkspringgreen!37}0.690 & \cellcolor{darkspringgreen!25}0.672 & 0.648 & \cellcolor{deepcarmine!48}0.589 & \cellcolor{deepcarmine!42}0.597 & \cellcolor{deepcarmine!48}0.589 & \cellcolor{deepcarmine!44}0.595 & \cellcolor{deepcarmine!38}0.604 & \cellcolor{deepcarmine!75}0.548 & \cellcolor{deepcarmine!35}0.609 \\ 
% 2016  & \cellcolor{darkspringgreen!60}\underline{0.717} & \cellcolor{darkspringgreen!67}\underline{0.725} & \cellcolor{darkspringgreen!29}0.677 & \underline{0.652} & \cellcolor{deepcarmine!12}\underline{0.649} & \cellcolor{deepcarmine!27}0.630 & \cellcolor{deepcarmine!38}0.616 & \cellcolor{deepcarmine!21}0.637 & \cellcolor{deepcarmine!75}0.569 & \cellcolor{deepcarmine!24}0.634 \\ 
% 2017  & \cellcolor{darkspringgreen!75}0.705 & \cellcolor{darkspringgreen!73}0.703 & \cellcolor{darkspringgreen!49}0.670 & \cellcolor{darkspringgreen!13}0.621 & 0.616 & \cellcolor{deepcarmine!17}0.606 & \cellcolor{deepcarmine!26}0.594 & \cellcolor{deepcarmine!17}0.606 & \cellcolor{deepcarmine!66}0.539 & \cellcolor{deepcarmine!12}0.613 \\ 
% 2018  & \cellcolor{darkspringgreen!75}0.693 & \cellcolor{darkspringgreen!68}0.685 & \cellcolor{darkspringgreen!48}0.658 & \cellcolor{deepcarmine!12}0.604 & \cellcolor{deepcarmine!11}0.605 & 0.607 & \cellcolor{deepcarmine!21}0.592 & \cellcolor{deepcarmine!19}0.595 & \cellcolor{deepcarmine!52}0.551 & \cellcolor{darkspringgreen!17}0.618 \\ 
% 2019  & \cellcolor{darkspringgreen!74}0.701 & \cellcolor{darkspringgreen!75}0.702 & \cellcolor{darkspringgreen!54}0.670 & \cellcolor{deepcarmine!10}0.603 & \cellcolor{darkspringgreen!19}0.618 & \cellcolor{darkspringgreen!12}0.607 & 0.603 & \cellcolor{deepcarmine!14}0.596 & \cellcolor{deepcarmine!59}0.527 & \cellcolor{darkspringgreen!13}0.608 \\ 
% 2020  & \cellcolor{darkspringgreen!70}0.716 & \cellcolor{darkspringgreen!75}0.722 & \cellcolor{darkspringgreen!54}\underline{0.695} & \cellcolor{darkspringgreen!10}0.635 & \cellcolor{darkspringgreen!10}0.635 & \cellcolor{deepcarmine!11}\underline{0.633} & \cellcolor{deepcarmine!18}\underline{0.624} & 0.635 & \cellcolor{deepcarmine!62}0.565 & \cellcolor{deepcarmine!16}0.627 \\ 
% 2021  & \cellcolor{darkspringgreen!75}0.705 & \cellcolor{darkspringgreen!72}0.698 & \cellcolor{darkspringgreen!57}0.664 & \cellcolor{darkspringgreen!34}0.609 & \cellcolor{darkspringgreen!39}0.622 & \cellcolor{darkspringgreen!34}0.609 & \cellcolor{darkspringgreen!30}0.600 & \cellcolor{darkspringgreen!41}0.625 & 0.552 & \cellcolor{darkspringgreen!49}\underline{0.645} \\ 
% 2022  & \cellcolor{darkspringgreen!75}0.716 & \cellcolor{darkspringgreen!71}0.712 & \cellcolor{darkspringgreen!47}0.685 & \cellcolor{deepcarmine!12}0.639 & \cellcolor{deepcarmine!12}0.639 & \cellcolor{deepcarmine!17}\underline{0.633} & \cellcolor{deepcarmine!27}0.622 & \cellcolor{deepcarmine!12}\underline{0.639} & \cellcolor{deepcarmine!72}\underline{0.570} & 0.642 \\ 
%         \bottomrule 
%         \end{tabular}} 
%         \caption{Accuracy@64 for \textit{shared} entities. The intensity of colours is organized by rows and represents \textbf{higher} and \textbf{lower} results. The best values for each column are underlined.} 
%         \label{ch_temporal_el:tab:general_table_new_entities}
% \end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Script to generate this table: 
% https://gitlab.ilabt.imec.be/kzaporoj/el_copenhagen/-/blob/main/src/wiki/wikipedia/jobs/models/s07_analyze_results_specific_year.py
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{table}
% \centering 
% \resizebox{0.5\columnwidth}{!} 
% {\begin{tabular}{l cc} 
%          \toprule 
%          Year & COVID related & Non-COVID related \\ 
%          \midrule
%          2021 & 0.4265 & 0.6510 \\
%         %  2022 & 0.6147 & 0.6482 \\
%         % \midrule 
%     \bottomrule 
% \end{tabular}} 
%     \caption{New entities in Wikipedia not always are associated with the new knowledge.} 
%     \label{ch_temporal_el:tab:covid_vs_non_covid}
% \end{table}

% \begin{table}[t] 
% \centering 
% \resizebox{1.0\columnwidth}{!} 
% {\begin{tabular}{l cccccccccc} 
%          \toprule 
%          & 2013 & 2014 & 2015 & 2016 & 2017 & 2018 & 2019 & 2020 & 2021 & 2022 \\ 
%         \midrule 
% 2013  & 0.759 & \cellcolor{deepcarmine!33}0.721 & \cellcolor{deepcarmine!69}0.663 & \cellcolor{deepcarmine!33}0.722 & \cellcolor{deepcarmine!43}0.705 & \cellcolor{deepcarmine!45}0.702 & \cellcolor{deepcarmine!30}0.727 & \cellcolor{deepcarmine!51}0.692 & \cellcolor{deepcarmine!75}0.655 & \cellcolor{deepcarmine!57}0.684 \\ 
% 2014  & - & - & - & - & - & - & - & - & - & - \\ 
% 2015  & \cellcolor{darkspringgreen!75}0.725 & \cellcolor{darkspringgreen!46}0.678 & 0.617 & \cellcolor{darkspringgreen!50}0.684 & \cellcolor{darkspringgreen!34}0.658 & \cellcolor{darkspringgreen!35}0.660 & \cellcolor{darkspringgreen!55}0.693 & \cellcolor{darkspringgreen!26}0.645 & \cellcolor{deepcarmine!14}0.609 & \cellcolor{darkspringgreen!21}0.636 \\ 
% 2016  & \cellcolor{darkspringgreen!59}0.758 & \cellcolor{deepcarmine!17}0.700 & \cellcolor{deepcarmine!66}0.650 & 0.708 & \cellcolor{deepcarmine!36}0.680 & \cellcolor{deepcarmine!36}0.681 & \cellcolor{darkspringgreen!28}0.726 & \cellcolor{deepcarmine!49}0.667 & \cellcolor{deepcarmine!75}0.642 & \cellcolor{deepcarmine!58}0.658 \\ 
% 2017  & - & - & - & - & - & - & - & - & - & - \\ 
% 2018  & - & - & - & - & - & - & - & - & - & - \\ 
% 2019  & \cellcolor{darkspringgreen!29}0.731 & \cellcolor{deepcarmine!24}0.688 & \cellcolor{deepcarmine!60}0.640 & \cellcolor{deepcarmine!19}0.694 & \cellcolor{deepcarmine!38}0.670 & \cellcolor{deepcarmine!38}0.669 & 0.706 & \cellcolor{deepcarmine!50}0.653 & \cellcolor{deepcarmine!75}0.622 & \cellcolor{deepcarmine!56}0.646 \\ 
% 2020  & - & - & - & - & - & - & - & - & - & - \\ 
% 2021  & \cellcolor{darkspringgreen!75}0.734 & \cellcolor{darkspringgreen!48}0.690 & \cellcolor{darkspringgreen!10}0.625 & \cellcolor{darkspringgreen!54}0.700 & \cellcolor{darkspringgreen!37}0.672 & \cellcolor{darkspringgreen!38}0.673 & \cellcolor{darkspringgreen!54}0.699 & \cellcolor{darkspringgreen!30}0.659 & 0.625 & \cellcolor{darkspringgreen!24}0.650 \\ 
% 2022  & - & - & - & - & - & - & - & - & - & - \\ 
%         \bottomrule 
%         \end{tabular}} 
%         \caption{Accuracy@64 for category random top 50 entities} 
%         \label{ch_temporal_el:tab:general_table_random_50}
% \end{table}

% \begin{table}[t]
% \centering
% \resizebox{0.9\columnwidth}{!}
% {\begin{tabular}{l cc c ccc c ccc}
%         \toprule
%          & \multicolumn{2}{c}{\#Entities} && \multicolumn{3}{c}{\#Mentions Shared} && \multicolumn{3}{c}{\#Mentions New} \\ 
%         \cmidrule(lr){2-3}\cmidrule(lr){5-7}\cmidrule(lr){9-11}
%         Cut & \ Shared & \ New && \# Train & \# Validation & \# Test && \# Train & \# Validation & \# Test \\ 
%         \midrule
%                 2013 & 10000 & 461 && 206847 & 216769 & 202707 && 2839 & 2141 & 2362 \\ 
%                 2014 & 10000 & 461 && 206850 & 216774 & 202708 && 2839 & 2141 & 2362 \\ 
%                 2015 & 10000 & 461 && 206850 & 216780 & 202707 && 2839 & 2141 & 2362 \\ 
%                 2016 & 10000 & 461 && 206852 & 216780 & 202710 && 2839 & 2141 & 2362 \\ 
%                 2017 & 10000 & 461 && 206852 & 216780 & 202711 && 2839 & 2141 & 2362 \\ 
%                 2018 & 10000 & 461 && 206850 & 216780 & 202710 && 2839 & 2141 & 2362 \\ 
%                 2019 & 10000 & 461 && 206851 & 216779 & 202708 && 2839 & 2141 & 2362 \\ 
%                 2020 & 10000 & 461 && 206854 & 216779 & 202708 && 2839 & 2141 & 2361 \\ 
%                 2021 & 10000 & 461 && 206854 & 216779 & 202708 && 2839 & 2141 & 2362 \\ 
%                 2022 & 10000 & 461 && 206854 & 216779 & 202709 && 2839 & 2141 & 2362 \\ 
%         \bottomrule
%         \end{tabular}}
%         \caption{Distribution across subsets.}
%         \label{ch_temporal_el:tab:dataset}
% \end{table}
% \begin{table}[t]
% \centering
% \resizebox{1.0\columnwidth}{!}
% {\begin{tabular}{l cccccccccc}
%         \toprule
%         & 2013 & 2014 & 2015 & 2016 & 2017 & 2018 & 2019 & 2020  & 2021  & 2022 \\ 
%         \midrule
%                 2013 & 0.000 & \cellcolor{deepcarmine!10}0.000 & \cellcolor{deepcarmine!15}0.000 & \cellcolor{deepcarmine!20}0.000 & \cellcolor{deepcarmine!25}0.000 & \cellcolor{deepcarmine!30}0.000 & \cellcolor{deepcarmine!35}0.000 & \cellcolor{deepcarmine!40}0.000 & \cellcolor{deepcarmine!45}0.000 & \cellcolor{deepcarmine!75}0.000 \\ 
%                 2014 & \cellcolor{deepcarmine!10}0.000 & 0.000 & \cellcolor{deepcarmine!10}0.000 & \cellcolor{deepcarmine!15}0.000 & \cellcolor{deepcarmine!20}0.000 & \cellcolor{deepcarmine!25}0.000 & \cellcolor{deepcarmine!30}0.000 & \cellcolor{deepcarmine!35}0.000 & \cellcolor{deepcarmine!40}0.000 & \cellcolor{deepcarmine!45}0.000 \\ 
%                 2015 & \cellcolor{deepcarmine!15}0.000 & \cellcolor{deepcarmine!10}0.000 & 0.000 & \cellcolor{deepcarmine!10}0.000 & \cellcolor{deepcarmine!15}0.000 & \cellcolor{deepcarmine!20}0.000 & \cellcolor{deepcarmine!25}0.000 & \cellcolor{deepcarmine!30}0.000 & \cellcolor{deepcarmine!35}0.000 & \cellcolor{darkspringgreen!75}0.000 \\ 
%                 2016 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\ 
%                 2017 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\ 
%                 2018 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\ 
%                 2019 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\ 
%                 2020 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\ 
%                 2021 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\ 
%                 2022 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\ 
%         \bottomrule
%         \end{tabular}}
%         \caption{Absolute accuracy or delta.}
%         \label{ch_temporal_el:tab:dataset}
% \end{table}
\section{Limitations and Future Work}
A number of dataset and model-related aspects were left unexplored in the current work. Clarifying them can help the community to understand the limitations and 
%to focus
% possible 
potential future research directions to extend our efforts. 

\noindent\textbf{Effect of pre-training on new corpora:} recent work has demonstrated the benefits of pre-training language models on more recent corpora (\eg latest Wikipedia versions) when applied on downstream tasks \cite{loureiro2022timelms, agarwal2021temporal}. We hypothesize some of these efforts can also be applicable to \ourdataset, specially to \textit{new} entities that often require additional knowledge to be correctly disambiguated. 

% \textbf{Continual learning models:} related with previous point .... \revklim{REF} complement fine-tuning as well as pre-training methods with continual learning, selectively adding new information... efficient ways of incorporating new knowledge in language models... 
% our dataset allows continual knowledge accumulation by adding the information on new entities/changes on existing ones... some citations here on adaptation.... 

% \textbf{Unique entity disambiguation:} due to limitation in resources .... cross encoder... due to limitation in resources.... couldn't extend it to more expressive (yet, also more expensive to train and evaluate) cross-encoder models. 

\noindent\textbf{Changes in mention context:} this work focused mostly on changes in target entities, leaving unexplored a study on how changes in mention context affect EL task. However, \figref{ch_temporal_el:fig:evolution_mentions} showcases a big drop in Jaccard vocabulary similarity of context around mentions, specially compared to immediately previous year. This suggests that the mentions, as well as the text surrounding them are highly volatile and evolving with time, making them an interesting subject for future research. 
% (\eg by analyzing the performance on \textit{shared} and \textit{new} entities). 
% Yet.... a future direction might be to understand better how the changes in entities or creation of new entities impact the creation or modification of the mentions/context around mentions.... 

\noindent\textbf{Cross-lingual time evolution:} our dataset is limited to English Wikipedia. Yet, recent work \cite{de2021multilingual,botha2020entity} has shown the benefits of training EL models in a cross-lingual setting. Thus, the study of cross-lingual temporal evolution of entity linking task appears to be an interesting future research direction.
% We group them in \textit{dataset-related} and \textit{model}
\section{Conclusions}
% We worked hard and achieved little 
This paper introduced \ourdataset, a first large-scale 
temporal
entity linking 
dataset 
composed of 10 yearly snapshots of Wikipedia target entities linked to by anchor mentions. We described the dataset creation pipeline, putting special focus on the quality assurance and future extensibility of \ourdataset. Furthermore, we experimented with the bi-encoder baseline model and showcased a consistent temporal deterioration in performance. We further examined the most challenging cases for this model, concluding the critical aspect of new knowledge acquisition during the pre-training phase. Finally, we described limitations of our work and discussed potential future research directions.
% to evaluate the temporal drift in performance of entity linking task.  
% We expect \ourdataset~will motivate a rise of entity disambiguation models that can address the evolutionary nature of the entity linking task. 
% \begin{ack}
% Thanks
% \end{ack}
% \section*{References}

% References follow the acknowledgments. Use unnumbered first-level heading for
% the references. Any choice of citation style is acceptable as long as you are
% consistent. It is permissible to reduce the font size to \verb+small+ (9 point)
% when listing the references.
% Note that the Reference section does not count towards the page limit.
% \medskip





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \appendix

% \section*{Appendix}
% \section{Appendix}
\newcounter{savechap}
\setcounter{savechap}{\value{chapter}}
\appendix
% \renewcommand*{\thesection}{\thechapter.\Alph{section}}
\renewcommand*{\thesection}{\thesavechap.\Alph{section}}
\section{Appendices}
% \addcontentsline{toc}{section}{Appendices}
% \renewcommand{\thesubsection}{\Alph{subsection}}
% \renewcommand{\thesubsection}{\thesection.\Alph{subsection}}
% \renewcommand{\thesubsection}{\thesection.\Alph{subsection}}

% Optionally include extra information (complete proofs, additional experiments and plots) in the appendix.
% This section will often be part of the supplemental material.
\subsection{Mentions per Entity Distribution}
\label{ch_temporal_el:app:mention_per_entity_distribution}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Script to generate these graph: 
% https://gitlab.ilabt.imec.be/kzaporoj/el_copenhagen/-/blob/main/src/wiki/wikipedia/jobs/dataset_creation/s04_final_dataset_statistics.py
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[!t]
\centering
% \includegraphics[width=1.0\columnwidth, trim={0.0cm 0.0cm 0.0cm 0.0cm},clip]{train_mentions_per_entity_20220512f.pdf}
\includegraphics[width=1.0\columnwidth, trim={0.0cm 0.0cm 0.0cm 0.0cm},clip]{s08_mentions_per_entity.pdf}
\caption{Distribution of the data across the temporal cuts. }
\label{ch_temporal_el:fig:men_entity_distribution}
\end{figure}
\Figref{ch_temporal_el:fig:men_entity_distribution} illustrates the equal mention per entity distribution across the temporal snapshots. This is achieved using weighted random sub-sampling (see \textit{Data Distributor} component description in \secref{ch_temporal_el:sec:dataset_construction}). 
% where the mentions pointing to entities with high number of incoming links have higher probability to be removed in snapshots with higher number of mentions. 
By enforcing this similarity between temporal snapshots, we ensure that the potential difference in the results is independent of cross-cut dataset distributional variations and only influenced by the dynamic temporal evolution of the content in \ourdataset. 
% (\eg given by changes in shared entities, creation of new entities, changes in the context of mentions, etc.). 
\subsection{Dataset Creation Hyperparameters}
\label{ch_temporal_el:app:hyperparameters}
\begin{table}[t]
\centering
\caption{Hyperparameters that can be tuned during \ourdataset~dataset creation. }
\label{ch_temporal_el:tab:hyperparameters}
{\renewcommand{\arraystretch}{1.2}
% \begin{tabular}{l lc}
\begin{tabular}{p{0.24\linewidth}  p{0.55\linewidth} c}
        \toprule
         Hyperparamter & \multicolumn{1}{c}{Description} & \ourdataset \\ 
         \midrule 
         \texttt{temporal\_cuts} & Details (\eg timestamps) of the temporal snapshots to be generated. & 10 years\footnotemark \\
         \texttt{nr\_sh\_ents\_per\_cut} & Number of shared entities per cut. & 10,000 \\
         \texttt{min\_mens\_per\_ent} & Minimum number of links a particular mention needs to have to target entity in order to be considered to be added in \ourdataset. & 1 \\
         \texttt{min\_men\_prior} & Minimum mention prior (see \equref{ch_temporal_el:eq:mention_prior}). & 0.0001 \\
         \texttt{max\_men\_prior} & Maximum mention prior. & 0.5 \\         
         \texttt{min\_men\_prior\_rank} & Minimum rank of mention prior among all the mentions pointing to a specific entity. & 2 \\
         \texttt{min\_ent\_prior} & Minimum entity prior as defined in \cite{yamada2016joint}. & 0.0 \\
         \texttt{max\_ent\_prior} & Maximum entity prior. & 1.0 \\
         \texttt{min\_nr\_inlinks} & Minimum number of incoming links per entity. & 10 \\
         \texttt{min\_len\_target\_ent} & Minimum length of target entity page (in tokens). & 10 \\
         \texttt{max\_mens\_per\_ent} & Maximum number of mentions per entity. & 500/10/10\footnotemark \\
         \texttt{ed\_men\_title} & Minimum normalized edit distance between the mentions and the title of the target page they are linked to. & 0.2 \\
         \texttt{ed\_men\_subsets} & Minimum normalized edit distance between the mentions in different subsets linked to the same target entity.  & 0.2 \\
         \bottomrule 
        \end{tabular}}
\end{table}
\footnotetext[8]{The actual format is different, indicating the timestamp of each of the temporal snapshots with up to a second of precision.}
\footnotetext[9]{For train, validation and test sets respectively.}
\Tabref{ch_temporal_el:tab:hyperparameters} summarizes the hyperparameters that can be tuned in order to automatically create the dataset. This way, it is possible for the user to create different variation of the \ourdataset. One example is by specifying different \texttt{temporal\_cuts} values to analyze the performance on other temporal periods (\eg monthly, quarterly, etc.).

\subsection{Mention and Entity Attributes}
\label{ch_temporal_el:app:mention_entity_attributes}
\begin{table}[t]
\centering
\caption{Attributes associated to each of the mention-entity pairs for each of the temporal cuts in \ourdataset. }
\label{ch_temporal_el:tab:attributes}
% {p{0.35\linewidth} | p{0.6\linewidth}}
{\renewcommand{\arraystretch}{1.2}
\begin{tabular}{p{0.26\linewidth}  p{0.68\linewidth}}
        \toprule
         Attribute & \multicolumn{1}{c}{Description} \\ 
         \midrule 
         \texttt{current\_snapshot} & The timestamp of the temporal snapshot from which the anchor mention and target entity attributes were extracted. \\
         \texttt{subset} & The name of current subset (\ie train, validation or test).\\
         \texttt{target\_text} & The textual content of the target entity Wikipedia page. \\
         \texttt{target\_len} & The length in tokens of target Wikipedia page. \\         
         \texttt{target\_title} & The title of target entity Wikipedia page. \\
         \texttt{category} & Category of the target entity (\textit{new} or \textit{shared}). \\         
         \texttt{mention\_text} & The text of the mention. \\
         \texttt{context\_left} & The textual context to the left of the mention. \\
         \texttt{context\_right} & The textual context to the right of the mention. \\
         \texttt{anchor\_len} & The length in tokens of the Wikipedia page where the anchor mention is located. \\
         \texttt{ed\_men\_title} & Normalized edit distance between the anchor mention and the title of the target Wikipedia page.  \\
         \texttt{overlap\_type} & Overlap type between the anchor mention and the target title as defined by \cite{logeswaran2019zero}. \\
         \texttt{men\_prior} & The mention prior (see \equref{ch_temporal_el:eq:mention_prior}). \\
         \texttt{men\_prior\_rank} & The rank of the current anchor mention compared to other mentions in Wikipedia pointing to target entity. \\
         \texttt{avg\_men\_prior} & The average value of prior of the mentions linked to the target entity in Wikipedia for \texttt{current\_snapshot}. \\
         \texttt{ent\_prior} & Entity prior as defined in \cite{yamada2016joint}. \\
         \texttt{nr\_inlinks} & Total number of incoming links to target entity. \\
         % \texttt{nr\_inlinks\_after\_fltr} & TODO \\
         \texttt{nr\_dist\_mens} & Number of distinct (\ie with different surface form) mentions linked to target entity. \\
         % \texttt{nr\_dist\_mens\_per\_cut\_per\_sset} & TODO \\
         \texttt{nr\_mens\_per\_ent} & Number of times the current mention appears in Wikipedia linked to target entity. \\ 
        %  \texttt{nr\_links\_per\_sset} & TODO \\
        %  \texttt{min\_nr\_links\_per\_sset} & TODO \\
         % \texttt{nr\_mens\_to\_extract\_per\_sset} & TODO \\
         \texttt{nr\_mens\_extracted} & Number of anchor mentions per current target entity in the \texttt{subset}. \\
         \texttt{anchor\_creation\_date} & The creation date (timestamp) of Wikipedia page where the anchor mention is located. \\
         \texttt{anchor\_revision\_date} & The timestamp of when the anchor Wikipedia page was last revised. \\
         \texttt{target\_creation\_date} & The timestamp of when the target Wikipedia entity page was created.  \\
         \texttt{target\_revision\_date} & The timestamp of when the target Wikipedia entity page was last modified. \\
         \bottomrule 
        \end{tabular}}
\end{table}
\Tabref{ch_temporal_el:tab:attributes} describes the anchor mention and target entity related attributes present in \ourdataset. These attributes can be used to perform more in-depth analysis of the results. 

\renewcommand{\labelenumi}{\arabic{enumi}.} % reset numbering
% {
% \small



\clearpage
\bibliographystyle{phdbib}
\bibliography{klim_ch_temporal_el/bibliography}
% }


% \renewcommand*{\thesection}{\thechapter.\arabic{section}}       % reset again to chaptnum.sectnum
% \bibliographystyle{phdbib}

% \bibliography{introbiblio}

% \bibliography{klim_ch_injecting/bibliography}

\clearpage{\pagestyle{empty}\cleardoublepage}


==> personal_data.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% document: personal_data.tex
%
% This file is intended to store the specific data of a PhD (e.g. title, promotor, author, scholarship etc) in order to keep the general template more generic.
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand\PhDauthor{Giannis Bekoulis}
\newcommand\PhDdomain{Computer Science Engineering}
\newcommand\PhDyear{2019--2020}
\newcommand\PhDDutchTitle{Neurale Benaderingen van Entiteitsgerichte Informatie-Extractie}
\newcommand\PhDEnglishTitle{Neural Approaches to Entity-Centric Information Extraction}%In English: Use Capitals for Each Word (except for words like: for, by, with, of, etc.)

\newboolean{PhDpromotorMultiple}
\setboolean{PhDpromotorMultiple}{true} %true if you have two promotors, false if you have only one
\newcommand\PhDpromotorFirst{prof.\ dr.\ ir.\ Chris Develder}%use lowercase for prof., dr. and ir.
\newcommand\PhDpromotorSecond{dr.\ ir.\ Thomas Demeester}

\newboolean{IWTscholarship}
\setboolean{IWTscholarship}{false} %true if you have an IWT scholarship, false if you don't
\newboolean{FWOscholarship}
\setboolean{FWOscholarship}{false} %true if you have an FWO scholarship, false if you don't

\hypersetup{											% this \hypersetup command adds metadata to your PDF document
 		pdftitle=\PhDEnglishTitle,    % title
    pdfauthor=\PhDauthor,     % author
    pdfsubject={PhD dissertation, Ghent University, Belgium},   % subject of the document
    %pdfcreator={Creator},   % creator of the document
    %pdfproducer={Producer}, % producer of the document
    %pdfkeywords={internet} {IBCN}, % list of keywords
    colorlinks,%
    citecolor=black,%
    filecolor=black,%
    linkcolor=black,%
    urlcolor=black
}





==> phdacronyms.tex <==
% List of Acronyms
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
{\makeatletter\gdef\reallynopagebreak{\par\nopagebreak\@nobreaktrue}}
\chapter*{List of Acronyms}


\reallynopagebreak
\begin{acronym}[HBCIHHH]


\acro{ADE}{Adverse Drug Events}
\acro{AI}{Artificial Intelligence}
\acro{AT}{Adversarial Training}
\acro{AVG}{Average}
\acro{BiLSTM}{Bidirectional LSTM}
\acro{BIO}{Beginning, Inside, Outside}
\acro{CBOW}{Continuous Bag-of-Words}
\acro{CRF}{Conditional Random Fields}
\acro{CNN}{Convolutional Neural Network}
\acro{DREC}{Dutch Real Estate Classifieds}
\acro{EC}{Entity Classification}
\acro{HMM}{Hidden Markov Model}
\acro{LSTM}{Long Short-Term Memory network}
\acro{LTM}{Locally Trained Model}
\acro{MTT}{Matrix-Tree Theorem}
\acro{MLP}{Multilayer Perceptron}
\acro{NER}{Named Entity Recognition}
\acro{NLP}{Natural Language Processing}
\acro{ORG}{Organization}
\acro{PER}{Person}
\acro{POS}{Part-of-Speech}
\acro{RE}{Relation Extraction}
\acro{RNN}{Recurrent Neural Network}
\acro{SVM}{Support Vector Machine}
\acro{TL}{Tweet-level LSTM}







\end{acronym}

% End of list of Acronyms
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> symbols.tex <==
% List of Symbols
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\chapter*{List of Symbols}

\begin{acronym_expdlist}
\acro{$b_m$}{bits per modulation symbol}
\acro{$BW$}{bandwidth [Hz]}
\acro{$c_r$}{the coding rate}
\acro{$T_s$}{OFDM symbol time [s]}
\end{acronym_expdlist}

% End of list of Symbols
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


